Adaptive stratified sampling for non-smooth problems

Science and engineering problems subject to uncertainty are frequently both computationally expensive and feature nonsmooth parameter dependence, making standard Monte Carlo too slow, and excluding efficient use of accelerated uncertainty quantification methods relying on strict smoothness assumptions. To remedy these challenges, we propose an adaptive stratification method suitable for nonsmooth problems and with significantly reduced variance compared to Monte Carlo sampling. The stratification is iteratively refined and samples are added sequentially to satisfy an allocation criterion combining the benefits of proportional and optimal sampling. Theoretical estimates are provided for the expected performance and probability of failure to correctly estimate essential statistics. We devise a practical adaptive stratification method with strata of the same kind of geometrical shapes, cost-effective refinement satisfying a greedy variance reduction criterion. Numerical experiments corroborate the theoretical findings and exhibit speedups of up to three orders of magnitude compared to standard Monte Carlo sampling.

==> basic-strat-samp-temp.tex <==
\section{Stratified Sampling Estimators} %: a few basics}
\label{sec:basic-strat-samp}
%{\color{red}
%  \begin{itemize}
%  \item take some details from the introduction
%  \item rewrite the linking text accordingly
%  \end{itemize}
%}


%To see that the resulting estimator of a quantity of interest indeed
%has lower variance compared to standard Monte Carlo sampling, let
%$\hat{f}$ denote an estimator of a statistic $f$, e.g., the
%expectation of a stochastic function. 

We assume that the quantity of
interest is the expectation of a scalar function $f$  on the domain
$\bX = (X_1,\dots, X_n) \in \mathbb{R}^{n}$, where the $X_k$
($k=1,\hdots,n$) are independent random variables with finite variance
and known but not necessarily identical probability distributions. By
means of the inverse Cumulative Distribution Function (CDF)
transformation, $X_k = F^{-1}_{X_k}(U_{k})$, where $U_k$ is a uniform
random variable on $[0, 1]$, and $F_{Y_i}$ denotes the CDF of
$X_{k}$. Without loss of generality, we may assume that the stochastic
domain is the hypercube $\Omega = [0,\ 1]^n$ and consider a
stratification $\mathcal{S}$ given by $\Omega = \cup_{ S\in\mathcal{S}} S$ of %$\Omega = \cup_{i=1}^{N_{\text{strata}}} S_{i}$ into
disjoint strata, i.e. $S \cap T = \emptyset$ if $S \neq T$. Then
$\mathbb{E}(f) = \sum_{S \in \mathcal{S}} p_{S} \mathbb{E}(f)$,
where $p_S$ is the probability measure of stratum $S$.  

---------------------

The stratification estimator $\hat{f}_{\text{strat}}$ of
$\mathbb{E}\bigl(f(\boldsymbol{X})\bigr)$ is
\begin{equation}
\label{eq:ss_estimator}
  \hat{f}_{\text{strat}} := \sum_{S\in\mathcal{S}}p_SE_{N_S}^{\text{mc}}\bigl(f(\boldsymbol{X}) \bigl.\bigr\vert \boldsymbol{X}\in S\bigr) \equiv \sum_{S\in\mathcal{S}}\frac{p_S}{N_S} \sum_{i=1}^{N_S}f\bigl(\boldsymbol{Z}_S^{(i)}\bigr)\;,
\end{equation}
%for a given stratification $\mathcal{S}$, 
where $\boldsymbol{Z}_S$ is
distributed according to the conditional distribution of
$\boldsymbol{X}$ given that $\boldsymbol{X}\in S$. {\color{red}[PP: How about using the notation $\bX_{S}$ for the conditional distribution (to avoid a new letter $Z$)?]} Moreover, let
$N:= \sum_{S\in\mathcal{S}} N_S$ denote the total number of
samples. 


---------------------

%The stratified
%sampling estimator is then given by
%\begin{equation}
%\label{eq:ss_estimator}
%\hat{f} = \sum_{i=1}^{N_{\text{strata}}} \frac{p_i}{N_i} \sum_{j=1}^{N_i} f(\bY_{S_i}^{(j)}),
%\end{equation}
%where $N_i$ is the number of samples in stratum $S_{i}$, and $\bY_{S_i}$ denotes the random vector $\bY$ conditional on $\bY \in S_i$. 
The estimator~\eqref{eq:ss_estimator} is unbiased and the proportion of samples in stratum $S$, denoted $q_{S} = N_{S}/N$ should be chosen to minimize the variance of the estimator.
Letting $\sigma_S$ denote the standard deviation of $f$ restricted to $S$,  the variance of the estimator~\eqref{eq:ss_estimator} is
\[
  \var{\hat{f}_{\text{strat}} } = \frac{1}{N} \sum_{ S \in \mathcal{S} } \frac{p_S^2 \sigma_S^2}{q_S}. 
\]
%%Proportional allocation $q_i = p_i$ yields a lower bound for the standard Monte Carlo estimate. Setting
%%\begin{equation}
%%\label{eq:opt_allo}
%%q_{i} = \frac{p_i \sigma_i}{\sum_{j=1}^{N_{\text{strata}}} p_j \sigma_j},
%%\end{equation}
%%leads to optimal allocation of samples, and the resulting estimator reaches the lower bound
%%\begin{equation}
%%%\label{eq:strat_var_lowb}
%%\var{\hat{f}}  = \frac{1}{N} \left( \sum_{i=1}^{N_{\text{strata}}} p_i \sigma_i \right)^{2}.
%%\end{equation}

%With the choice~\eqref{eq:opt_allo} for the proportions of samples within each strata, the variance is minimized. 


%-------------------------

\begin{equation*}
  \var{\hat{f}_{\text{strat}} } = \sum_{S\in\mathcal{S}}{\mathbb{P}(\boldsymbol{X}\in S)}^2 \frac{\var{f(\boldsymbol{X}) \bigl.\bigr\vert \boldsymbol{X}\in S}}{N_S} = \sum_{S\in\mathcal{S}}{\mathbb{P}(\boldsymbol{X}\in S)}^2 \frac{\var{f(\boldsymbol{Z}_S)}}{N_S}
\end{equation*}

  The expression above is independent of the sample allocation
  rule for the number of samples per stratum $N_S$. In practice, there
  are two popular rules, namely proportional allocation
  \begin{equation*}
    N^{\text{prop}}_S := p_S N\;,
  \end{equation*}
  and optimal sample allocation
  \begin{equation}
  \label{eq:opt_allo}
    N^{\text{opt}}_S := \frac{p_S\sigma_S}{\sum_{S\in \mathcal{S}}p_S \sigma_S} N\;,
  \end{equation}
  where, as before,
  $\sigma_S \equiv \sqrt{\mu_2(S)} :=
  \sqrt{\var{f(\boldsymbol{Z}_S)}}$ denotes the conditional (output)
  standard deviation in stratum $S$. The latter allocation rule is
  optimal in the sense that it provides the stratification estimator
  with the smallest variance amongst all stratification estimators for
  a given stratification $\mathcal{S}$. In fact, the corresponding
  estimator variances are
\begin{align}
\label{eq:strat_var_lowb}
  \mathcal{V}_{\text{opt}} &:= \var{\left.\hat{f}_{\text{strat}}\right\vert_{N_S = N^{\text{opt}}_S}} = \frac{1}{N} {\Bigl(\sum_{S\in\mathcal{S}}p_S \sigma_S\Bigr)}^2\;,
\\
  \mathcal{V}_{\text{prop}} &:= \var{\left.\hat{f}_{\text{strat}}\right\vert_{N_S = N^{\text{prop}}_S}} = \frac{1}{N} \sum_{S\in\mathcal{S}}p_S \sigma_S^2\;,
\end{align}
respectively. These choices of sample allocations both assume that the the stratum variances are known, which would not be the case in practical situations. An algorithm to adaptively allocate samples to asymptotically achieve the lower bound~\eqref{eq:strat_var_lowb} was introduced in~\cite{Etore_Jourdain_10}. Adaptive stratified sampling based on adjustment of strata via a stratification matrix was investigated in~\cite{Etore_etal_11}.



%-------------------------



Stratified sampling is usually restricted to low dimensions due to exponential growth in the number of strata with increasing dimension. This problem can be overcome by using, e.g., latin hypercube sampling where only the marginal distributions are stratified~\cite{Kroese_etal_11}. In this work, we propose adaptivity in the dynamic stratification of the stochastic domain as a means to reduce the total number of strata created.


%%%%%%%%%%%%%


While the previous subsection addressed the failure to identify a high
variance region, the main goal in practice is to quantify the
performance of the adaptive stratification estimator. Recall that the
adaption is motivated to maintain an effective variance reduction even
in the presence of heterogeneous features. That is, the adaptive
iterative procedure outlined above yields, roughly
speaking,\footnote{{\color{red}[restate as remark at a later stage]}
  Actually, I think it will not possible to make this really exact, as
  we will have dependencies on the previously sampled variables. To
  overcome this, one could use $N/2$ samples to learn the
  stratification. Then fix the obtained stratification and use the
  remaining $N/2$ as in usual stratification estimator. However, to be
  fair, we will then have to compare the variance reduction of our
  method using $N/2$ samples with Monte Carlo using N samples. } a
stratification of the sampling domain, so that the estimator at the
final iteration can be viewed a classic stratification estimator. The
crucial difference is, of course, that its stratification has been
adapted to the problem at hand.  Nonetheless, given a stratification,
the theoretical results available for classic stratification
estimators apply here; see. e.g., \cite[Ch.~V,
Sect.~7]{Asmussen_Glynn_07}. %Recall that the stratification estimator is given by [[]]
%-----------------
%To be more precise, recall that the
%stratification estimator $\hat{f}_{\text{strat}}$ of
%$\mathbb{E}\bigl(f(\boldsymbol{X})\bigr)$ is
%\begin{equation*}
%  \hat{f}_{\text{strat}} := \sum_{S\in\mathcal{S}}p_SE_{N_S}^{\text{mc}}\bigl(f(\boldsymbol{X}) \bigl.\bigr\vert \boldsymbol{X}\in S\bigr) \equiv \sum_{S\in\mathcal{S}}\frac{p_S}{N_S} \sum_{i=1}^{N_S}f\bigl(\boldsymbol{Z}_S^{(i)}\bigr)\;,
%\end{equation*}
%for a given stratification $\mathcal{S}$, where $\boldsymbol{Z}_S$ is
%distributed according to the conditional distribution of
%$\boldsymbol{X}$ given that $\boldsymbol{X}\in S$. Moreover, let
%$N:= \sum_{S\in\mathcal{S}} N_S$ denote the total number of
%samples. 
%-----------------
For a given stratification $\mathcal{S}$ the estimator
$\hat{f}_{\text{strat}}$ given by~\eqref{eq:ss_estimator} is unbiased, i.e.,
\begin{equation*}
  \mathbb{E}\bigl( \hat{f}_{\text{strat}} \bigr) = \sum_{S\in\mathcal{S}}\mathbb{P}(\boldsymbol{X}\in S) \mathbb{E}\bigl(f(\boldsymbol{X}) \bigl.\bigr\vert \boldsymbol{X}\in S\bigr) = \mathbb{E}\bigl( f(\boldsymbol{X})\bigr),
\end{equation*}
and its variance is given by [[]]
%\begin{equation*}
%  \var{\hat{f}_{\text{strat}} } = \sum_{S\in\mathcal{S}}{\mathbb{P}(\boldsymbol{X}\in S)}^2 \frac{\var{f(\boldsymbol{X}) \bigl.\bigr\vert \boldsymbol{X}\in S}}{N_S} = \sum_{S\in\mathcal{S}}{\mathbb{P}(\boldsymbol{X}\in S)}^2 \frac{\var{f(\boldsymbol{Z}_S)}}{N_S}
%\end{equation*}
for any number of samples per strata $N_S$,
$S\in\mathcal{S}$. Moreover, if $N_S$ is such that
$\lim_{N\to\infty}\frac{N}{N_S} < \infty$, then
$\lim_{N\to\infty} N \var{\hat{f}_{\text{strat}} } < \infty$ and
$\hat{f}_{\text{strat}}$ satisfies the central limit theorem
\begin{equation*}
  \frac{\hat{f}_{\text{strat}} - \mathbb{E}\bigl( f(\boldsymbol{X})\bigr) }{\sqrt{\var{\hat{f}_{\text{strat}} }} } \underset{N\to\infty}{\Rightarrow}\mathcal{N}(0,1)\;.
\end{equation*}
In practice when $N\gg 1$, this asymptotic normality can thus be used
to not only report a point estimate for
$\mathbb{E}\bigl( f(\boldsymbol{X})\bigr)$ (i.e., simply the obtained
value $\hat{f}_{\text{strat}}$), also an approximate confidence
region. For example, let $q_{1-\alpha/2}$ be the $1-\alpha/2$ quantile
of the standard normal distribution so that 
\begin{equation*}
  \begin{aligned}
    1-\alpha &\approx \mathbb{P}\left( {\var{\hat{f}_{\text{strat}} }}^{-1/2}\left\vert \hat{f}_{\text{strat}} - \mathbb{E}\bigl( f(\boldsymbol{X})\bigr) \right\vert \le q_{1-\alpha/2}\right)\\
    &= \mathbb{P}\left( \hat{f}_{\text{strat}} -  q_{1-\alpha/2} \sqrt{\var{\hat{f}_{\text{strat}} }} \le \mathbb{E}\bigl( f(\boldsymbol{X})\bigr) \le  \hat{f}_{\text{strat}} +  q_{1-\alpha/2} \sqrt{\var{\hat{f}_{\text{strat}} }}\right)\;.
  \end{aligned}
  \end{equation*}
  In other words: the unknown value
  $\mathbb{E}\bigl( f(\boldsymbol{X})\bigr)$ is contained in the
  confidence interval
  \begin{equation*}
    I_{\alpha} := \left[ \hat{f}_{\text{strat}} -  q_{1-\alpha/2}\sqrt{\var{\hat{f}_{\text{strat}} }}  , \hat{f}_{\text{strat}} +  q_{1-\alpha/2}  \sqrt{\var{\hat{f}_{\text{strat}} }}\right]
  \end{equation*}
  with probability approximately equal to $1-\alpha$.
%
  An alternative approach to quantifying the probability of failure is, in view of Chebyshev's inequality:
  \begin{equation*}
    \mathbb{P} \Bigl(\bigl\vert\hat{f}_{\text{strat}} - \mathbb{E}\bigl( f(\boldsymbol{X})\bigr) \bigr\vert \ge \theta \Bigr) \le \frac{\var{\hat{f}_{\text{strat}} }}{\theta^2}\;,
  \end{equation*}
  for any $\theta>0$. While this estimate does not rely on an
  asymptotic normality assumption, it may be not as sharp as the
  corresponding statement based on a normal approximation if $N\gg 1$.

  What both estimates have in common is that they are controlled by
  the estimator's variance. However, for these approaches to be
  practical, we require an accurate estimation of the stratification
  estimator's standard deviation or variance. Next, we will quantify
  the probability of misestimating the standard
  deviation. 

  \subsection{Quantifying the accuracy of the variance estimators}
  
  Although the sampling allocation $N_S = N^{\text{opt}}_S$ yields the
stratification estimator with minimal variance, the optimal allocation
rule requires the standard deviations $\sigma_S$ for all
$S\in\mathcal{S}$ to be known. In practice this is, of course, not
feasible and the standard deviations $\sigma_S$ are estimated by the
empirical standard deviation $\hat{\sigma}_S$ in each stratum.
 Given a stratification $\mathcal{S}$, the natural
variance estimators in practice thus are
\begin{equation*}
  \hat{V}_{\text{prop}} := \frac{1}{N} \sum_{S\in\mathcal{S}}p_S \hat{\sigma}_S^2
  \quad\text{and}\quad
  \hat{V}_{\text{opt}} := \frac{1}{N} {\Bigl(\sum_{S\in\mathcal{S}}p_S \hat{\sigma}_S\Bigr)}^2\;,
\end{equation*}
where $\hat{\sigma}^2_S := h_2(S)$ and $\hat{\sigma}_S := \sqrt{h_2(S)}$
denote the empirical variance and empirical standard deviation in
stratum $S$, respectively, based on $N_S $ samples. This approximation may, however,
have practical limitations, because $\hat{\sigma}_S$ is not an unbiased estimator for
the standard deviation $\sigma_S$. In fact, $\hat{\sigma}_S$ is only
an asymptotically unbiased estimator in contrast to
$\hat{\sigma}^2_S$, which is an unbiased estimator for the
variance. The Lemma below gives probabilistic bounds for quantifying
the deviations of both the stratification estimator's standard
deviation and variance estimates from the theorized values, that also
account for this induced estimation bias in every stratum.
%
\begin{lemma}[Optimal sample allocation]
  For a given stratification $\mathcal{S}$, let
  $\hat{f}_{\text{strat}}$ be the stratification estimator with
  $N_S = N^{\text{opt}}_S$ samples in each stratum
  $S\in\mathcal{S}$. Suppose that for every stratum $S\in\mathcal{S}$
  there exist constants $0\le m_S\le M_S$, such that
  $m_S \le \hat\sigma_S \le M_S$ almost surely. Then
  \begin{equation*}
    \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}_{\text{opt}}} - \sqrt{\mathcal{V}_{\text{opt}}} \bigr\vert \ge \theta \Bigr)
    \le 2 \exp{\left(-\frac{2{\left(\lvert B_1\rvert - \theta\sqrt{N}\right)}^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;,
  \end{equation*}
  for any $\theta >\frac{\lvert B_1\rvert}{\sqrt{N}}$, where
  $B_1 := \sum_{S\in\mathcal{S}} p_S b_S$ and
  $b_S := \mathbb{E}(\hat\sigma_S) - \sigma_S$ for
  $S\in\mathcal{S}$. Moreover, it holds that
  \begin{equation*}
    \mathbb{P}\Bigl(\bigl\vert \hat{V}_{\text{opt}} - \mathcal{V}_{\text{opt}} \bigr\vert \ge \vartheta \Bigr)
    \le 2 \exp{\left(-\frac{2{\left(\lvert B_2\rvert - \vartheta N\right)}^2}{{\left(\sum_{S\in\mathcal{S}} p_S M_S\right)}^4}\right)}\;,
  \end{equation*}
  for any $\vartheta >\frac{\lvert B_2\rvert}{N}$, where
  $B_2 := \sum_{S,T\in\mathcal{S}, S\not= T}p_S p_T \bigl(b_S b_T + b_S \sigma_T + b_T \sigma_S\bigr)$.
\end{lemma}
\begin{proof}
  Let $\hat{V} \equiv \hat{V}_{\text{opt}}$ and
  $\mathcal{V} \equiv \mathcal{V}_{\text{opt}}$, and
  $\theta\ge0$. Then
  \begin{equation*}
    \begin{aligned}
      \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
      &=  \mathbb{P}\Bigl(\Bigl\vert \sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S) \Bigr\vert \ge \theta \sqrt{N}\Bigr)\\
      &= \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S)  \ge \theta \sqrt{N}\Bigr) +
    \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S)  \le -\theta \sqrt{N}\Bigr)\\
    & =: P_1 + P_2\;.
  \end{aligned}
\end{equation*}
It follows from Markov's inequality that $P_1$ and $P_2$ can be bounded by 
\begin{equation*}
  P_1 \le e^{-t\theta\sqrt{N} }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{t(\hat\sigma_S - \sigma_S)p_S}\bigr)\;,\quad\text{and}\quad
  P_2 \le e^{-t\theta\sqrt{N} }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{-t(\hat\sigma_S - \sigma_S)p_S}\bigr)\;,
\end{equation*}
respectively, for any $t>0$, where we have used the fact that
$\hat\sigma_{S}$ and $\hat\sigma_{T}$ are independent for strata
$S, T\in\mathcal{S}$ if $S\not= T$. Moreover, in view of Hoeffding's
lemma and the hypotheses we then find that
\begin{equation*}
  \prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{\pm t(\hat\sigma_S - \sigma_S)p_S}\bigr) \le \prod_{S\in\mathcal{S}} e^{\pm tp_S b_S + t^2 {p_S}^2 \frac{{(M_S - m_S)}^2}{8}}
  = e^{\pm t B_1 + \frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\;,
\end{equation*}
where $B_1 := \sum_{S\in\mathcal{S}} p_S b_S$ and
$b_S := \mathbb{E}(\hat\sigma_S) - \sigma_S$. Using these upper bounds
with the bounds for $P_1$ and $P_2$ we we eventually obtain
\begin{equation*}
  \begin{aligned}
    \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
    &\le e^{-t\theta\sqrt{N} + \frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2} \Bigl( e^{ t B_1}
    + e^{-t B_1}\Bigr)\\
    & \le 2 e^{\frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2 + t\left(\lvert B_1\rvert - \theta\sqrt{N}\right)}\;,
  \end{aligned}
\end{equation*}
for any $t>0$. Minimizing the right-hand side then yields
\begin{equation*}
    \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
    \le 2 \exp{\left(-\frac{2{\left(\lvert B_1\rvert - \theta\sqrt{N}\right)}^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;,
\end{equation*}
provided that $\theta > \lvert B_1\rvert/\sqrt{N}$, and thus the
claim.
% The claim for the standard deviation's relative error follows
% immideatiely from the above upon using
% $\theta = \tau \sqrt{\mathcal{V}} \equiv \tau \varsigma/\sqrt{N}$ for
% a suitable $\tau\ge 0$. Indeed, letting 
% $R := \sqrt{\hat{V}/\mathcal{V}}$, then
% \eqref{eq:failure:prob:global:hoeffding:abs:final} can be restated as
% \begin{equation}\label{eq:failure:prob:global:hoeffding:rel:final}
%     \mathbb{P}\bigl(\lvert R - 1 \rvert \ge \tau \bigr)
%     \le 2 \exp{\left(-\frac{2{\left(\lvert B_1\rvert - \tau\varsigma\right)}^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;,
% \end{equation}
% provided that
% \begin{equation*}
%   \tau > \frac{\lvert B_1\rvert}{\varsigma}\;.
% \end{equation*}

The proof of the variance bound is similar to the proof for the standard deviation above. Indeed, let $\vartheta\ge
0$, then
\begin{equation*}
    \begin{aligned}
      \mathbb{P}\Bigl(\bigl\vert \hat{V} - \mathcal{V} \bigr\vert \ge \vartheta \Bigr)
      &=  \mathbb{P}\Bigl(\sum_{S,T\in\mathcal{S}}p_S p_T(\hat\sigma_S\hat\sigma_T - \sigma_S\sigma_T) \ge \vartheta N\Bigr) + \mathbb{P}\Bigl(\sum_{S,T\in\mathcal{S}}p_S p_T(\hat\sigma_S\hat\sigma_T - \sigma_S\sigma_T) \le -\vartheta N\Bigr)\\
      &=: P_1 + P_2\;.
  \end{aligned}
\end{equation*}
Markov's inequality yields
\begin{equation*}
  P_1 \le e^{-t\vartheta N }\mathbb{E}\Bigl( e^{t \sum_{S,T\in\mathcal{S}}p_S p_T(\hat\sigma_S\hat\sigma_T - \sigma_S\sigma_T)} \Bigr)\quad\text{and}\quad
  P_2 \le e^{-t\vartheta N }\mathbb{E}\Bigl( e^{-t \sum_{S,T\in\mathcal{S}}p_S p_T(\hat\sigma_S\hat\sigma_T - \sigma_S\sigma_T)} \Bigr)
\end{equation*}
for any $t>0$. Although we cannot exploit the independence of
$\hat\sigma_S$ across strata that easily, we can still proceed as
before. In fact, here Hoeffding's lemma yields
\begin{equation*}
  \mathbb{E}\Bigl( e^{\pm t \sum_{S,T\in\mathcal{S}}p_S p_T(\hat\sigma_S\hat\sigma_T - \sigma_S\sigma_T)} \Bigr)
  \le e^{\pm t B_2 + \frac{t^2}{8} {\left(\sum_{S\in\mathcal{S}} p_S M_S\right)}^4}
\end{equation*}
using the fact that 
\begin{equation*}
  -{\Bigl(\sum_{S\in\mathcal{S}} p_S \sigma_S\Bigr)}^2\le  N\bigl(\hat{V} - \mathcal{V}\bigr) \le
{\Bigl(\sum_{S\in\mathcal{S}} p_S M_S\Bigr)}^2 -
{\Bigl(\sum_{S\in\mathcal{S}} p_S \sigma_S\Bigr)}^2\;.
\end{equation*}
 Here, the bias $B_2$ is
\begin{equation*}
  B_2 := \sum_{S,T\in\mathcal{S}, S\not= T}p_S p_T \bigl(b_S b_T + b_S \sigma_T + b_T \sigma_S\bigr)\;,
\end{equation*}
with $b_S$ as before. Combining these estimates yields
\begin{equation*}
  \mathbb{P}\Bigl(\bigl\vert \hat{V} - \mathcal{V} \bigr\vert \ge \vartheta \Bigr)
  \le \min_{t>0} 2 e^{t \left(\lvert B_2\rvert - \vartheta N\right) + \frac{t^2}{8} {\left(\sum_{S\in\mathcal{S}} p_S M_S\right)}^4}
  = 2 \exp{\left(-\frac{2{\left(\lvert B_2\rvert - \vartheta N\right)}^2}{{\left(\sum_{S\in\mathcal{S}} p_S M_S\right)}^4}\right)}\;,
\end{equation*}
provided that $\vartheta > \lvert B_2\rvert/N$.
\end{proof}

\begin{remark}
  We reiterate that the standard deviation estimator's bias
  $\delta_S = \mathbb{E}(\hat\sigma_S) - \sigma_S$ is not zero,
  despite the fact that $\hat\sigma_S^2 \equiv h_2(S)$ is an unbiased
  estimator of $\mu_2(S) \equiv \sigma_S^2$. This is essentially due
  to the non-linearity of the square root. In fact, it is known that
  $\delta(S)= \mathcal{O}(1/N_S)$ and, moreover, that one cannot find
  an empirical standard deviation estimator that is unbiased for all
  distributions. {\color{red} REFs}
\end{remark}

In contrast, the stratification estimator using a proportional sample
allocation may not offer the biggest variance reduction but the
accuracy of its natural variance estimate is unaffected by a biased
standard deviation estimation in the strata.
% 
\begin{lemma}[Proportional allocation]
  For a stratification $\mathcal{S}$, let $\hat{f}_{\text{strat}}$ be
  the stratification estimator with $N_S = N^{\text{prop}}_S$ samples
  in each stratum $S\in\mathcal{S}$. Suppose that for every stratum
  $S\in\mathcal{S}$ there exist constants $0\le m_S\le M_S$, such that
  $m_S \le \hat\sigma_S \le M_S$ almost surely. Then
  \begin{equation*}
  \mathbb{P}\Bigl(\bigl\vert \hat{V}_{\text{prop}} - \mathcal{V}_{\text{prop}} \bigr\vert \ge \vartheta \Bigr)
  \le 2 \exp{\left(- \frac{2 \vartheta^2 N^2}{\sum_{S\in\mathcal{S}} {p_S}^2 {({M_S}^2-{m_S}^2)}^2}\right)}\;,
\end{equation*}
for any $\vartheta > 0$.
\end{lemma}
\begin{proof}
  We proceed as in the proof for the standard deviation
  above. Therefore, let $\hat{V} \equiv \hat{V}_{\text{prop}}$ and
  $\mathcal{V} \equiv \mathcal{V}_{\text{prop}}$, and
  $\vartheta\ge0$. Then
  \begin{equation*}
    \begin{aligned}
      \mathbb{P}\Bigl(\bigl\vert \hat{V} - \mathcal{V} \bigr\vert \ge \vartheta \Bigr)
      &= \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S({\hat\sigma_S}^2 - \sigma^2_S)  \ge \vartheta N\Bigr) +
    \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S({\hat\sigma_S}^2 - \sigma^2_S)  \le -\vartheta N\Bigr)\\
    & =: P_1 + P_2\;.
  \end{aligned}
\end{equation*}
It follows  that
\begin{equation*}
  P_1 \le e^{-t\vartheta N }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{t({\hat\sigma_S}^2 - \sigma_S)p_S}\bigr)\;,\quad\text{and}\quad
  P_2 \le e^{-t\vartheta N }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{-t({\hat\sigma_S}^2 - \sigma_S)p_S}\bigr)\;,
\end{equation*}
for any $t>0$. Together with Hoeffding's
lemma and the hypotheses we thus find
\begin{equation*}
  P1 + P2 \le 2 e^{\frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{({M_S}^2 - {m_S}^2)}^2 - t\vartheta N}\;.
\end{equation*}
Minimizing the right-hand side over $t>0$ eventually yields the claim.
\end{proof}

{\color{red}
Interpretation as relative error?
$\varsigma_{\text{opt}}:= N \mathcal{V}_{\text{opt}}$ and 
$\varsigma_{\text{prop}}:= N \mathcal{V}_{\text{prop}}$
}


\subsection{Asymptotic variance reduction}

{\color{red}
  [Can add theoretical results from slides on the effect of allocation rules for continuous and discontinuous functions here?]}

Introduce \emph{variance reduction factor}
        \begin{equation*}
          \mathfrak{R}_{\text{str},\ast} := N
          \var{\bigl(\hat{Q}_{\ast}\bigr)}\;,\quad \ast\in\{\text{prop},\text{opt}\}\;,
        \end{equation*}
        for each allocation rule.

Effect of allocation rule, which is an extension of a result by {\scriptsize [Asmussen and Glynn. 2007]}.
    

\begin{lemma}[{Asymptotic variance reduction}]
    Consider a uniform stratification
    $\mathcal{S}$ of $\mathfrak{U}\subset\mathbb{R}^n$. If $f\in C^1(\mathfrak{U})$, then
    \begin{equation*}
        \mathfrak{R}_{\text{str},\text{prop}} \le C_{\text{prop}}\, {\lvert \mathcal{S}\rvert}^{-\frac{2}{n}}\quad\text{and}\quad
        \mathfrak{R}_{\text{str},\text{opt}} \le C_{\text{opt}}\, {\lvert \mathcal{S}\rvert}^{-\frac{2}{n}}\;,
    \end{equation*}
    with $C_{\text{prop}}$ and $C_{\text{opt}}$ independent of the
    stratification $\mathcal{S}$.

    Conversely, if $f\colon \mathfrak{U}\to\mathbb{R}$ is piecewise
    constant with a jump discontinuity across a curve $\Gamma$ in
    $\mathfrak{U}$ and the set of strata
    $\mathcal{T}\subset\mathcal{S}$ containing $\Gamma$ satisfies
    $\lvert \mathcal{T}\rvert = \mathcal{O}({\lvert
      \mathcal{S}\rvert}^\frac{n-1}{n})$, then
    \begin{equation*}
      \mathfrak{R}_{\text{str},\text{prop}} \le \hat{C}_{\text{prop}}\, {\lvert \mathcal{S}\rvert}^{-\frac{1}{n}}\quad\text{and}\quad
        \mathfrak{R}_{\text{str},\text{opt}} \le \hat{C}_{\text{opt}}\, {\lvert \mathcal{S}\rvert}^{-\frac{2}{n}}\;,
      \end{equation*}%
    with $\hat{C}_{\text{prop}}$ and $\hat{C}_{\text{opt}}$ independent of the
    stratification $\mathcal{S}$.
\end{lemma}


\begin{proof}
  Direct computation using the mean value theorem and Cauchy--Schwarz ineq.
   \end{proof}

   Notice that the preceeding lemma states that at last asymptoticall,
   optimal allocation not superior to proportional allocation for
   smooth problems.


   \begin{figure}
        \centering
        \includegraphics[width=0.25\textwidth]{../presentation/figs_strat_basics/discont_uniform}\quad
        \includegraphics[width=0.25\textwidth]{../presentation/figs_strat_basics/discont_adaptive}
        \caption{hello}
      \end{figure}

   


summary: robust and sub-optimal vs.\ volataile and optimal

% {\color{gray}
% That is, let
% $\theta\ge0$, then the probability of misestimating the true standard
% deviation by $\theta$ is
% \begin{equation}\label{eq:failure:prob:global:abs}
%   \begin{aligned}
%     \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
%     &=  \mathbb{P}\Bigl(\Bigl\vert \sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S) \Bigr\vert \ge \theta \sqrt{N}\Bigr)\\
%     &= \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S)  \ge \theta \sqrt{N}\Bigr) +
%     \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S)  \le -\theta \sqrt{N}\Bigr)\\
%     & =: P_1 + P_2\;.
%   \end{aligned}
% \end{equation}
% It follows from Markov's inequality that $P_1$ and $P_2$ can be bounded by 
% \begin{equation*}
%   P_1 \le e^{-t\theta\sqrt{N} }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{t(\hat\sigma_S - \sigma_S)p_S}\bigr)\;,\quad\text{and}\quad
%   P_2 \le e^{-t\theta\sqrt{N} }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{-t(\hat\sigma_S - \sigma_S)p_S}\bigr)\;,
% \end{equation*}
% respectively, for any $t>0$, where we have used the fact that
% $\hat\sigma_{S_1}$ and $\hat\sigma_{S_2}$ are independent for strata
% $S_1, S_2\in\mathcal{S}$ if $S_1\not= S_2$. Putting both estimates
% together and minimizing over $t>0$, we find the upper bound for the
% failure probability as
% \begin{equation}
%   \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
%   \le \min_{t>0}e^{-t\theta\sqrt{N} }\left(\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{t(\hat\sigma_S - \sigma_S)p_S}\bigr) + \prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{-t(\hat\sigma_S - \sigma_S)p_S}\bigr)\right)\;.\label{eq:failure:prob:global:hoeffding:abs}
% \end{equation}
% For certain functions $f$ it may be possible to deduce the
% distribution of $Y_S := f(\boldsymbol{Z}_S)$, and thus also of
% $\hat\sigma_S = \sqrt{h_2(S)}$,\footnote{Or making a Gaussian
%   approximation...} which may allow to compute the moment generating
% function $\tau\mapsto \mathbb{E}(e^{\tau\hat\sigma_S})$ in closed
% form. However, this does not seem to be the case in general. On the
% other hand, if $0\le \hat\sigma_S$ is almost surely bounded, then we
% can use Hoeffding's lemma to derive more insightful estimates. Indeed,
% such a boundedness assumption seems reasonable, in particular when
% assuming that $f$ does not contain any singularities in $S$. In fact,
% if $-\infty< l_S := \inf_S f \le \sup_S f =: u_S <\infty$, then
% $h_2(S) \le \frac{N}{N-1}({u_S}^2 - {l_S}^2) \le 2({u_S}^2 - {l_S}^2)
% $. We thus suppose that $0\le m_S\le \hat\sigma_S\le M_S$ almost
% surely on stratum $S$. In view of Hoeffding's lemma we then find
% \begin{equation*}
%   \prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{\pm t(\hat\sigma_S - \sigma_S)p_S}\bigr) \le \prod_{S\in\mathcal{S}} e^{\pm tp_S\delta(S) + t^2 {p_S}^2 \frac{{(M_S - m_S)}^2}{8}}
%   = e^{\pm t\sum_{S\in\mathcal{S}} p_S \delta(S) + \frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\;,
% \end{equation*}
% where $\delta(S) := \mathbb{E}(\hat\sigma_S) - \sigma_S$ denotes the
% bias of the empirical standard deviation estimator
% $\hat\sigma_S = \sqrt{h_2(S)}$. Notice that $\delta(S)$ is not zero,
% despite the fact that $\hat\sigma_S^2 \equiv h_2(S)$ is an unbiased
% estimator of $\mu_2(S) \equiv \sigma_S^2$ due to the non-linearity of
% the square root. In fact, it is known that
% $\delta(S)= \mathcal{O}(1/N_S)$ and, moreover, that one cannot find an
% empirical standard deviation estimator that is unbiased for all
% distributions. Using the upper bound in
% \eqref{eq:failure:prob:global:hoeffding:abs}, we eventually obtain
% \begin{equation}\label{eq:failure:prob:global:hoeffding:abs:final}
%   \begin{aligned}
%     \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
%     &\le \min_{t>0} e^{-t\theta\sqrt{N} + \frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2} \Bigl( e^{ t\sum_{S\in\mathcal{S}} p_S \delta(S)}
%     + e^{-t\sum_{S\in\mathcal{S}} p_S \delta(S)}\Bigr)\\
%     & \le 2 \min_{t>0} e^{\frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2 + t\left(\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert - \theta\sqrt{N}\right)}\\
%     & = 2 \exp{\left(-\frac{2{\left(\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert - \theta\sqrt{N}\right)}^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;,
%   \end{aligned}
% \end{equation}
% provided that
% \begin{equation*}
%   \theta > \frac{1}{\sqrt{N}} \sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert\;.
% \end{equation*}
% Notice that the bound
% \eqref{eq:failure:prob:global:hoeffding:abs:final} also offers an
% estimate for the relative error, which provides insight into the
% effect of the given stratification alone. To see this, set
% $R := \sqrt{\hat{V}/\mathcal{V}}$ and use
% $\theta = \tau \sqrt{\mathcal{V}} \equiv \tau
% \varsigma/\sqrt{N}$ for a suitable $\tau\ge 0$, where
% $\varsigma := \sum_{S\in\mathcal{S}}p_S \sigma_S$. Then
% \eqref{eq:failure:prob:global:hoeffding:abs:final} can be restated as
% \begin{equation}\label{eq:failure:prob:global:hoeffding:rel:final}
%     \mathbb{P}\bigl(\lvert R - 1 \rvert \ge \tau \bigr)
%     \le 2 \exp{\left(-\frac{2{\left(\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert - \tau\varsigma\right)}^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;,
% \end{equation}
% provided that
% \begin{equation*}
%   \tau > \frac{\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert}{\varsigma}
%   = \frac{\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert}{\sum_{S\in\mathcal{S}} p_S\sigma_S}\;.
% \end{equation*}

% }




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Master"
%%% End:

==> basic-strat-samp.tex <==
\section{Stratified Sampling Estimators} %: a few basics}
\label{sec:basic-strat-samp}
%{\color{red}
%  \begin{itemize}
%  \item take some details from the introduction
%  \item rewrite the linking text accordingly
%  \end{itemize}
%}


%To see that the resulting estimator of a quantity of interest indeed
%has lower variance compared to standard Monte Carlo sampling, let
%$\hat{f}$ denote an estimator of a statistic $f$, e.g., the
%expectation of a stochastic function. 

We assume that the quantity of
interest is the expectation of a scalar function $f$  on the domain
$\bY = (Y_1,\dots, Y_n) \in \mathbb{R}^{n}$, where the $Y_k$
($k=1,\hdots,n$) are independent random variables with finite variance
and known but not necessarily identical probability distributions. By
means of the inverse Cumulative Distribution Function (CDF)
transformation, $Y_k = F^{-1}_{Y_k}(U_{k})$, where $U_k$ is a uniform
random variable on $[0, 1]$, and $F_{Y_i}$ denotes the CDF of
$Y_{k}$. Without loss of generality, we may assume that the stochastic
domain is the hypercube $\Omega = [0,\ 1]^n$ and consider a
stratification $\Omega = \cup_{i=1}^{N_{\text{strata}}} S_{i}$ into
disjoint strata $S_{i} \cap S_{j} = \emptyset$ if $i\neq j$. Then
$\mathbb{E}(f) = \sum_{i=1}^{N_{\text{strata}}} p_{i} \mathbb{E}(f)$,
where $p_i$ is the probability measure of stratum $i$.  

---------------------

The stratification estimator $\hat{f}_{\text{strat}}$ of
$\mathbb{E}\bigl(f(\boldsymbol{X})\bigr)$ is
\begin{equation}
\label{eq:ss_estimator}
  \hat{f}_{\text{strat}} := \sum_{S\in\mathcal{S}}p_SE_{N_S}^{\text{mc}}\bigl(f(\boldsymbol{X}) \bigl.\bigr\vert \boldsymbol{X}\in S\bigr) \equiv \sum_{S\in\mathcal{S}}\frac{p_S}{N_S} \sum_{i=1}^{N_S}f\bigl(\boldsymbol{Z}_S^{(i)}\bigr)\;,
\end{equation}
for a given stratification $\mathcal{S}$, where $\boldsymbol{Z}_S$ is
distributed according to the conditional distribution of
$\boldsymbol{X}$ given that $\boldsymbol{X}\in S$. Moreover, let
$N:= \sum_{S\in\mathcal{S}} N_S$ denote the total number of
samples. 


---------------------

%The stratified
%sampling estimator is then given by
%\begin{equation}
%\label{eq:ss_estimator}
%\hat{f} = \sum_{i=1}^{N_{\text{strata}}} \frac{p_i}{N_i} \sum_{j=1}^{N_i} f(\bY_{S_i}^{(j)}),
%\end{equation}
%where $N_i$ is the number of samples in stratum $S_{i}$, and $\bY_{S_i}$ denotes the random vector $\bY$ conditional on $\bY \in S_i$. 
The estimator~\eqref{eq:ss_estimator} is unbiased and the proportion of samples in stratum $S_i$, denoted $q_{i} = N_{i}/N$ should be chosen to minimize the variance of the estimator.
Letting $\sigma_i$ denote the standard deviation of $f$ restricted to $S_i$,  the variance of the estimator~\eqref{eq:ss_estimator} is
\[
\var{\hat{f}} = \frac{1}{N} \sum_{i=1}^{N_{\text{strata}}} \frac{p_i^2 \sigma_i^2}{q_i}. 
\]
%%Proportional allocation $q_i = p_i$ yields a lower bound for the standard Monte Carlo estimate. Setting
%%\begin{equation}
%%\label{eq:opt_allo}
%%q_{i} = \frac{p_i \sigma_i}{\sum_{j=1}^{N_{\text{strata}}} p_j \sigma_j},
%%\end{equation}
%%leads to optimal allocation of samples, and the resulting estimator reaches the lower bound
%%\begin{equation}
%%%\label{eq:strat_var_lowb}
%%\var{\hat{f}}  = \frac{1}{N} \left( \sum_{i=1}^{N_{\text{strata}}} p_i \sigma_i \right)^{2}.
%%\end{equation}

%With the choice~\eqref{eq:opt_allo} for the proportions of samples within each strata, the variance is minimized. 


%-------------------------

\begin{equation*}
  \var{\hat{f}_{\text{strat}} } = \sum_{S\in\mathcal{S}}{\mathbb{P}(\boldsymbol{X}\in S)}^2 \frac{\var{f(\boldsymbol{X}) \bigl.\bigr\vert \boldsymbol{X}\in S}}{N_S} = \sum_{S\in\mathcal{S}}{\mathbb{P}(\boldsymbol{X}\in S)}^2 \frac{\var{f(\boldsymbol{Z}_S)}}{N_S}
\end{equation*}

  The expression above is independent of the sample allocation
  rule for the number of samples per stratum $N_S$. In practice, there
  are two popular rules, namely proportional allocation
  \begin{equation*}
    N^{\text{prop}}_S := p_S N\;,
  \end{equation*}
  and optimal sample allocation
  \begin{equation}
  \label{eq:opt_allo}
    N^{\text{opt}}_S := \frac{p_S\sigma_S}{\sum_{S\in \mathcal{S}}p_S \sigma_S} N\;,
  \end{equation}
  where, as before,
  $\sigma_S \equiv \sqrt{\mu_2(S)} :=
  \sqrt{\var{f(\boldsymbol{Z}_S)}}$ denotes the conditional (output)
  standard deviation in stratum $S$. The latter allocation rule is
  optimal in the sense that it provides the stratification estimator
  with the smallest variance amongst all stratification estimators for
  a given stratification $\mathcal{S}$. In fact, the corresponding
  estimator variances are
\begin{align}
\label{eq:strat_var_lowb}
  \mathcal{V}_{\text{opt}} &:= \var{\left.\hat{f}_{\text{strat}}\right\vert_{N_S = N^{\text{opt}}_S}} = \frac{1}{N} {\Bigl(\sum_{S\in\mathcal{S}}p_S \sigma_S\Bigr)}^2\;,
\\
  \mathcal{V}_{\text{prop}} &:= \var{\left.\hat{f}_{\text{strat}}\right\vert_{N_S = N^{\text{prop}}_S}} = \frac{1}{N} \sum_{S\in\mathcal{S}}p_S \sigma_S^2\;,
\end{align}
respectively. These choices of sample allocations both assume that the the stratum variances are known, which would not be the case in practical situations. An algorithm to adaptively allocate samples to asymptotically achieve the lower bound~\eqref{eq:strat_var_lowb} was introduced in~\cite{Etore_Jourdain_10}. Adaptive stratified sampling based on adjustment of strata via a stratification matrix was investigated in~\cite{Etore_etal_11}.



%-------------------------



Stratified sampling is usually restricted to low dimensions due to exponential growth in the number of strata with increasing dimension. This problem can be overcome by using, e.g., latin hypercube sampling where only the marginal distributions are stratified~\cite{Kroese_etal_11}. In this work, we propose adaptivity in the dynamic stratification of the stochastic domain as a means to reduce the total number of strata created.


%%%%%%%%%%%%%


While the previous subsection addressed the failure to identify a high
variance region, the main goal in practice is to quantify the
performance of the adaptive stratification estimator. Recall that the
adaption is motivated to maintain an effective variance reduction even
in the presence of heterogeneous features. That is, the adaptive
iterative procedure outlined above yields, roughly
speaking,\footnote{{\color{red}[restate as remark at a later stage]}
  Actually, I think it will not possible to make this really exact, as
  we will have dependencies on the previously sampled variables. To
  overcome this, one could use $N/2$ samples to learn the
  stratification. Then fix the obtained stratification and use the
  remaining $N/2$ as in usual stratification estimator. However, to be
  fair, we will then have to compare the variance reduction of our
  method using $N/2$ samples with Monte Carlo using N samples. } a
stratification of the sampling domain, so that the estimator at the
final iteration can be viewed a classic stratification estimator. The
crucial difference is, of course, that its stratification has been
adapted to the problem at hand.  Nonetheless, given a stratification,
the theoretical results available for classic stratification
estimators apply here; see. e.g., \cite[Ch.~V,
Sect.~7]{Asmussen_Glynn_07}. %Recall that the stratification estimator is given by [[]]
%-----------------
%To be more precise, recall that the
%stratification estimator $\hat{f}_{\text{strat}}$ of
%$\mathbb{E}\bigl(f(\boldsymbol{X})\bigr)$ is
%\begin{equation*}
%  \hat{f}_{\text{strat}} := \sum_{S\in\mathcal{S}}p_SE_{N_S}^{\text{mc}}\bigl(f(\boldsymbol{X}) \bigl.\bigr\vert \boldsymbol{X}\in S\bigr) \equiv \sum_{S\in\mathcal{S}}\frac{p_S}{N_S} \sum_{i=1}^{N_S}f\bigl(\boldsymbol{Z}_S^{(i)}\bigr)\;,
%\end{equation*}
%for a given stratification $\mathcal{S}$, where $\boldsymbol{Z}_S$ is
%distributed according to the conditional distribution of
%$\boldsymbol{X}$ given that $\boldsymbol{X}\in S$. Moreover, let
%$N:= \sum_{S\in\mathcal{S}} N_S$ denote the total number of
%samples. 
%-----------------
For a given stratification $\mathcal{S}$ the estimator
$\hat{f}_{\text{strat}}$ given by~\eqref{eq:ss_estimator} is unbiased, i.e.,
\begin{equation*}
  \mathbb{E}\bigl( \hat{f}_{\text{strat}} \bigr) = \sum_{S\in\mathcal{S}}\mathbb{P}(\boldsymbol{X}\in S) \mathbb{E}\bigl(f(\boldsymbol{X}) \bigl.\bigr\vert \boldsymbol{X}\in S\bigr) = \mathbb{E}\bigl( f(\boldsymbol{X})\bigr),
\end{equation*}
and its variance is given by [[]]
%\begin{equation*}
%  \var{\hat{f}_{\text{strat}} } = \sum_{S\in\mathcal{S}}{\mathbb{P}(\boldsymbol{X}\in S)}^2 \frac{\var{f(\boldsymbol{X}) \bigl.\bigr\vert \boldsymbol{X}\in S}}{N_S} = \sum_{S\in\mathcal{S}}{\mathbb{P}(\boldsymbol{X}\in S)}^2 \frac{\var{f(\boldsymbol{Z}_S)}}{N_S}
%\end{equation*}
for any number of samples per strata $N_S$,
$S\in\mathcal{S}$. Moreover, if $N_S$ is such that
$\lim_{N\to\infty}\frac{N}{N_S} < \infty$, then
$\lim_{N\to\infty} N \var{\hat{f}_{\text{strat}} } < \infty$ and
$\hat{f}_{\text{strat}}$ satisfies the central limit theorem
\begin{equation*}
  \frac{\hat{f}_{\text{strat}} - \mathbb{E}\bigl( f(\boldsymbol{X})\bigr) }{\sqrt{\var{\hat{f}_{\text{strat}} }} } \underset{N\to\infty}{\Rightarrow}\mathcal{N}(0,1)\;.
\end{equation*}
In practice when $N\gg 1$, this asymptotic normality can thus be used
to not only report a point estimate for
$\mathbb{E}\bigl( f(\boldsymbol{X})\bigr)$ (i.e., simply the obtained
value $\hat{f}_{\text{strat}}$), also an approximate confidence
region. For example, let $q_{1-\alpha/2}$ be the $1-\alpha/2$ quantile
of the standard normal distribution so that 
\begin{equation*}
  \begin{aligned}
    1-\alpha &\approx \mathbb{P}\left( {\var{\hat{f}_{\text{strat}} }}^{-1/2}\left\vert \hat{f}_{\text{strat}} - \mathbb{E}\bigl( f(\boldsymbol{X})\bigr) \right\vert \le q_{1-\alpha/2}\right)\\
    &= \mathbb{P}\left( \hat{f}_{\text{strat}} -  q_{1-\alpha/2} \sqrt{\var{\hat{f}_{\text{strat}} }} \le \mathbb{E}\bigl( f(\boldsymbol{X})\bigr) \le  \hat{f}_{\text{strat}} +  q_{1-\alpha/2} \sqrt{\var{\hat{f}_{\text{strat}} }}\right)\;.
  \end{aligned}
  \end{equation*}
  In other words: the unknown value
  $\mathbb{E}\bigl( f(\boldsymbol{X})\bigr)$ is contained in the
  confidence interval
  \begin{equation*}
    I_{\alpha} := \left[ \hat{f}_{\text{strat}} -  q_{1-\alpha/2}\sqrt{\var{\hat{f}_{\text{strat}} }}  , \hat{f}_{\text{strat}} +  q_{1-\alpha/2}  \sqrt{\var{\hat{f}_{\text{strat}} }}\right]
  \end{equation*}
  with probability approximately equal to $1-\alpha$.
%
  An alternative approach to quantifying the probability of failure is, in view of Chebyshev's inequality:
  \begin{equation*}
    \mathbb{P} \Bigl(\bigl\vert\hat{f}_{\text{strat}} - \mathbb{E}\bigl( f(\boldsymbol{X})\bigr) \bigr\vert \ge \theta \Bigr) \le \frac{\var{\hat{f}_{\text{strat}} }}{\theta^2}\;,
  \end{equation*}
  for any $\theta>0$. While this estimate does not rely on an
  asymptotic normality assumption, it may be not as sharp as the
  corresponding statement based on a normal approximation if $N\gg 1$.

  What both estimates have in common is that they are controlled by
  the estimator's variance. However, for these approaches to be
  practical, we require an accurate estimation of the stratification
  estimator's standard deviation or variance. Next, we will quantify
  the probability of misestimating the standard
  deviation. 

  \subsection{Quantifying the accuracy of the variance estimators}
  
  Although the sampling allocation $N_S = N^{\text{opt}}_S$ yields the
stratification estimator with minimal variance, the optimal allocation
rule requires the standard deviations $\sigma_S$ for all
$S\in\mathcal{S}$ to be known. In practice this is, of course, not
feasible and the standard deviations $\sigma_S$ are estimated by the
empirical standard deviation $\hat{\sigma}_S$ in each stratum.
 Given a stratification $\mathcal{S}$, the natural
variance estimators in practice thus are
\begin{equation*}
  \hat{V}_{\text{prop}} := \frac{1}{N} \sum_{S\in\mathcal{S}}p_S \hat{\sigma}_S^2
  \quad\text{and}\quad
  \hat{V}_{\text{opt}} := \frac{1}{N} {\Bigl(\sum_{S\in\mathcal{S}}p_S \hat{\sigma}_S\Bigr)}^2\;,
\end{equation*}
where $\hat{\sigma}^2_S := h_2(S)$ and $\hat{\sigma}_S := \sqrt{h_2(S)}$
denote the empirical variance and empirical standard deviation in
stratum $S$, respectively, based on $N_S $ samples. This approximation may, however,
have practical limitations, because $\hat{\sigma}_S$ is not an unbiased estimator for
the standard deviation $\sigma_S$. In fact, $\hat{\sigma}_S$ is only
an asymptotically unbiased estimator in contrast to
$\hat{\sigma}^2_S$, which is an unbiased estimator for the
variance. The Lemma below gives probabilistic bounds for quantifying
the deviations of both the stratification estimator's standard
deviation and variance estimates from the theorized values, that also
account for this induced estimation bias in every stratum.
%
\begin{lemma}[Optimal sample allocation]
  For a given stratification $\mathcal{S}$, let
  $\hat{f}_{\text{strat}}$ be the stratification estimator with
  $N_S = N^{\text{opt}}_S$ samples in each stratum
  $S\in\mathcal{S}$. Suppose that for every stratum $S\in\mathcal{S}$
  there exist constants $0\le m_S\le M_S$, such that
  $m_S \le \hat\sigma_S \le M_S$ almost surely. Then
  \begin{equation*}
    \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}_{\text{opt}}} - \sqrt{\mathcal{V}_{\text{opt}}} \bigr\vert \ge \theta \Bigr)
    \le 2 \exp{\left(-\frac{2{\left(\lvert B_1\rvert - \theta\sqrt{N}\right)}^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;,
  \end{equation*}
  for any $\theta >\frac{\lvert B_1\rvert}{\sqrt{N}}$, where
  $B_1 := \sum_{S\in\mathcal{S}} p_S b_S$ and
  $b_S := \mathbb{E}(\hat\sigma_S) - \sigma_S$ for
  $S\in\mathcal{S}$. Moreover, it holds that
  \begin{equation*}
    \mathbb{P}\Bigl(\bigl\vert \hat{V}_{\text{opt}} - \mathcal{V}_{\text{opt}} \bigr\vert \ge \vartheta \Bigr)
    \le 2 \exp{\left(-\frac{2{\left(\lvert B_2\rvert - \vartheta N\right)}^2}{{\left(\sum_{S\in\mathcal{S}} p_S M_S\right)}^4}\right)}\;,
  \end{equation*}
  for any $\vartheta >\frac{\lvert B_2\rvert}{N}$, where
  $B_2 := \sum_{S,T\in\mathcal{S}, S\not= T}p_S p_T \bigl(b_S b_T + b_S \sigma_T + b_T \sigma_S\bigr)$.
\end{lemma}
\begin{proof}
  Let $\hat{V} \equiv \hat{V}_{\text{opt}}$ and
  $\mathcal{V} \equiv \mathcal{V}_{\text{opt}}$, and
  $\theta\ge0$. Then
  \begin{equation*}
    \begin{aligned}
      \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
      &=  \mathbb{P}\Bigl(\Bigl\vert \sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S) \Bigr\vert \ge \theta \sqrt{N}\Bigr)\\
      &= \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S)  \ge \theta \sqrt{N}\Bigr) +
    \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S)  \le -\theta \sqrt{N}\Bigr)\\
    & =: P_1 + P_2\;.
  \end{aligned}
\end{equation*}
It follows from Markov's inequality that $P_1$ and $P_2$ can be bounded by 
\begin{equation*}
  P_1 \le e^{-t\theta\sqrt{N} }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{t(\hat\sigma_S - \sigma_S)p_S}\bigr)\;,\quad\text{and}\quad
  P_2 \le e^{-t\theta\sqrt{N} }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{-t(\hat\sigma_S - \sigma_S)p_S}\bigr)\;,
\end{equation*}
respectively, for any $t>0$, where we have used the fact that
$\hat\sigma_{S}$ and $\hat\sigma_{T}$ are independent for strata
$S, T\in\mathcal{S}$ if $S\not= T$. Moreover, in view of Hoeffding's
lemma and the hypotheses we then find that
\begin{equation*}
  \prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{\pm t(\hat\sigma_S - \sigma_S)p_S}\bigr) \le \prod_{S\in\mathcal{S}} e^{\pm tp_S b_S + t^2 {p_S}^2 \frac{{(M_S - m_S)}^2}{8}}
  = e^{\pm t B_1 + \frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\;,
\end{equation*}
where $B_1 := \sum_{S\in\mathcal{S}} p_S b_S$ and
$b_S := \mathbb{E}(\hat\sigma_S) - \sigma_S$. Using these upper bounds
with the bounds for $P_1$ and $P_2$ we we eventually obtain
\begin{equation*}
  \begin{aligned}
    \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
    &\le e^{-t\theta\sqrt{N} + \frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2} \Bigl( e^{ t B_1}
    + e^{-t B_1}\Bigr)\\
    & \le 2 e^{\frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2 + t\left(\lvert B_1\rvert - \theta\sqrt{N}\right)}\;,
  \end{aligned}
\end{equation*}
for any $t>0$. Minimizing the right-hand side then yields
\begin{equation*}
    \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
    \le 2 \exp{\left(-\frac{2{\left(\lvert B_1\rvert - \theta\sqrt{N}\right)}^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;,
\end{equation*}
provided that $\theta > \lvert B_1\rvert/\sqrt{N}$, and thus the
claim.
% The claim for the standard deviation's relative error follows
% immideatiely from the above upon using
% $\theta = \tau \sqrt{\mathcal{V}} \equiv \tau \varsigma/\sqrt{N}$ for
% a suitable $\tau\ge 0$. Indeed, letting 
% $R := \sqrt{\hat{V}/\mathcal{V}}$, then
% \eqref{eq:failure:prob:global:hoeffding:abs:final} can be restated as
% \begin{equation}\label{eq:failure:prob:global:hoeffding:rel:final}
%     \mathbb{P}\bigl(\lvert R - 1 \rvert \ge \tau \bigr)
%     \le 2 \exp{\left(-\frac{2{\left(\lvert B_1\rvert - \tau\varsigma\right)}^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;,
% \end{equation}
% provided that
% \begin{equation*}
%   \tau > \frac{\lvert B_1\rvert}{\varsigma}\;.
% \end{equation*}

The proof of the variance bound is similar to the proof for the standard deviation above. Indeed, let $\vartheta\ge
0$, then
\begin{equation*}
    \begin{aligned}
      \mathbb{P}\Bigl(\bigl\vert \hat{V} - \mathcal{V} \bigr\vert \ge \vartheta \Bigr)
      &=  \mathbb{P}\Bigl(\sum_{S,T\in\mathcal{S}}p_S p_T(\hat\sigma_S\hat\sigma_T - \sigma_S\sigma_T) \ge \vartheta N\Bigr) + \mathbb{P}\Bigl(\sum_{S,T\in\mathcal{S}}p_S p_T(\hat\sigma_S\hat\sigma_T - \sigma_S\sigma_T) \le -\vartheta N\Bigr)\\
      &=: P_1 + P_2\;.
  \end{aligned}
\end{equation*}
Markov's inequality yields
\begin{equation*}
  P_1 \le e^{-t\vartheta N }\mathbb{E}\Bigl( e^{t \sum_{S,T\in\mathcal{S}}p_S p_T(\hat\sigma_S\hat\sigma_T - \sigma_S\sigma_T)} \Bigr)\quad\text{and}\quad
  P_2 \le e^{-t\vartheta N }\mathbb{E}\Bigl( e^{-t \sum_{S,T\in\mathcal{S}}p_S p_T(\hat\sigma_S\hat\sigma_T - \sigma_S\sigma_T)} \Bigr)
\end{equation*}
for any $t>0$. Although we cannot exploit the independence of
$\hat\sigma_S$ across strata that easily, we can still proceed as
before. In fact, here Hoeffding's lemma yields
\begin{equation*}
  \mathbb{E}\Bigl( e^{\pm t \sum_{S,T\in\mathcal{S}}p_S p_T(\hat\sigma_S\hat\sigma_T - \sigma_S\sigma_T)} \Bigr)
  \le e^{\pm t B_2 + \frac{t^2}{8} {\left(\sum_{S\in\mathcal{S}} p_S M_S\right)}^4}
\end{equation*}
using the fact that 
\begin{equation*}
  -{\Bigl(\sum_{S\in\mathcal{S}} p_S \sigma_S\Bigr)}^2\le  N\bigl(\hat{V} - \mathcal{V}\bigr) \le
{\Bigl(\sum_{S\in\mathcal{S}} p_S M_S\Bigr)}^2 -
{\Bigl(\sum_{S\in\mathcal{S}} p_S \sigma_S\Bigr)}^2\;.
\end{equation*}
 Here, the bias $B_2$ is
\begin{equation*}
  B_2 := \sum_{S,T\in\mathcal{S}, S\not= T}p_S p_T \bigl(b_S b_T + b_S \sigma_T + b_T \sigma_S\bigr)\;,
\end{equation*}
with $b_S$ as before. Combining these estimates yields
\begin{equation*}
  \mathbb{P}\Bigl(\bigl\vert \hat{V} - \mathcal{V} \bigr\vert \ge \vartheta \Bigr)
  \le \min_{t>0} 2 e^{t \left(\lvert B_2\rvert - \vartheta N\right) + \frac{t^2}{8} {\left(\sum_{S\in\mathcal{S}} p_S M_S\right)}^4}
  = 2 \exp{\left(-\frac{2{\left(\lvert B_2\rvert - \vartheta N\right)}^2}{{\left(\sum_{S\in\mathcal{S}} p_S M_S\right)}^4}\right)}\;,
\end{equation*}
provided that $\vartheta > \lvert B_2\rvert/N$.
\end{proof}

\begin{remark}
  We reiterate that the standard deviation estimator's bias
  $\delta_S = \mathbb{E}(\hat\sigma_S) - \sigma_S$ is not zero,
  despite the fact that $\hat\sigma_S^2 \equiv h_2(S)$ is an unbiased
  estimator of $\mu_2(S) \equiv \sigma_S^2$. This is essentially due
  to the non-linearity of the square root. In fact, it is known that
  $\delta(S)= \mathcal{O}(1/N_S)$ and, moreover, that one cannot find
  an empirical standard deviation estimator that is unbiased for all
  distributions. {\color{red} REFs}
\end{remark}

In contrast, the stratification estimator using a proportional sample
allocation may not offer the biggest variance reduction but the
accuracy of its natural variance estimate is unaffected by a biased
standard deviation estimation in the strata.
% 
\begin{lemma}[Proportional allocation]
  For a stratification $\mathcal{S}$, let $\hat{f}_{\text{strat}}$ be
  the stratification estimator with $N_S = N^{\text{prop}}_S$ samples
  in each stratum $S\in\mathcal{S}$. Suppose that for every stratum
  $S\in\mathcal{S}$ there exist constants $0\le m_S\le M_S$, such that
  $m_S \le \hat\sigma_S \le M_S$ almost surely. Then
  \begin{equation*}
  \mathbb{P}\Bigl(\bigl\vert \hat{V}_{\text{prop}} - \mathcal{V}_{\text{prop}} \bigr\vert \ge \vartheta \Bigr)
  \le 2 \exp{\left(- \frac{2 \vartheta^2 N^2}{\sum_{S\in\mathcal{S}} {p_S}^2 {({M_S}^2-{m_S}^2)}^2}\right)}\;,
\end{equation*}
for any $\vartheta > 0$.
\end{lemma}
\begin{proof}
  We proceed as in the proof for the standard deviation
  above. Therefore, let $\hat{V} \equiv \hat{V}_{\text{prop}}$ and
  $\mathcal{V} \equiv \mathcal{V}_{\text{prop}}$, and
  $\vartheta\ge0$. Then
  \begin{equation*}
    \begin{aligned}
      \mathbb{P}\Bigl(\bigl\vert \hat{V} - \mathcal{V} \bigr\vert \ge \vartheta \Bigr)
      &= \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S({\hat\sigma_S}^2 - \sigma^2_S)  \ge \vartheta N\Bigr) +
    \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S({\hat\sigma_S}^2 - \sigma^2_S)  \le -\vartheta N\Bigr)\\
    & =: P_1 + P_2\;.
  \end{aligned}
\end{equation*}
It follows  that
\begin{equation*}
  P_1 \le e^{-t\vartheta N }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{t({\hat\sigma_S}^2 - \sigma_S)p_S}\bigr)\;,\quad\text{and}\quad
  P_2 \le e^{-t\vartheta N }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{-t({\hat\sigma_S}^2 - \sigma_S)p_S}\bigr)\;,
\end{equation*}
for any $t>0$. Together with Hoeffding's
lemma and the hypotheses we thus find
\begin{equation*}
  P1 + P2 \le 2 e^{\frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{({M_S}^2 - {m_S}^2)}^2 - t\vartheta N}\;.
\end{equation*}
Minimizing the right-hand side over $t>0$ eventually yields the claim.
\end{proof}

{\color{red}
Interpretation as relative error?
$\varsigma_{\text{opt}}:= N \mathcal{V}_{\text{opt}}$ and 
$\varsigma_{\text{prop}}:= N \mathcal{V}_{\text{prop}}$
}


\subsection{Asymptotic variance reduction}



Introduce \emph{variance reduction factor}

Recall that 
        
        for each allocation rule.

Effect of allocation rule, which is an extension of a result by {\scriptsize [Asmussen and Glynn. 2007]}.
    

\begin{lemma}[{Asymptotic variance reduction}]
  Consider a uniform hyperrectangluar stratification $\mathcal{S}$ of
  $\mathfrak{U}\subset\mathbb{R}^n$ and let $Q := f(\bY)$ for some
  suitable function $f\colon\mathfrak{U}\to\mathbb{R}$.

  If $f\in C^1(\mathfrak{U})$, then the variance of the stratification
  estimator $\hat{Q}_{\alpha}$ satisfies
    \begin{equation*}
      \var{\hat{Q}_{\alpha}} \le \frac{n C}{3\, N}\, {\lvert \mathcal{S} \rvert}^{-2/n}
         \min\left(\frac{1}{\alpha}, \frac{1}{1-\alpha}\right)\;,
     \end{equation*}
     for any $\alpha\in[0,1]$, where
     $C = \sup_{\bu\in\mathfrak{U}}\Vert \nabla f(\bu)\Vert_2^2 \le
     \Vert f\Vert_{C^1(\mathfrak{U})}^2$.

     If $f\colon \mathfrak{U}\to\mathbb{R}$ is a piecewise
     constant function with a jump discontinuity of size $\delta>0$
     across a ($n-1$ dimensional) curve $\Gamma$ in $\mathfrak{U}$,
     then the stratification estimator's variance is bounded by
     \begin{equation*}
       \var{\hat{Q}_{\alpha}} \le \frac{\delta^2}{4\,N}
       \begin{cases}
         \frac{\lvert \mathcal{T} \rvert}{\lvert \mathcal{S} \rvert}\;,& \alpha = 0\;,\\
         \frac{\lvert \mathcal{T}\rvert}{\lvert \mathcal{S}\rvert}\, \min\left\{\frac{1}{1-\alpha}, \frac{1}{\alpha}\, \frac{\lvert \mathcal{T}\rvert}{\lvert \mathcal{S}\rvert}\right\}\;,& 0<\alpha < 1 \;,\\
         {\left(\frac{\lvert \mathcal{T} \rvert}{\lvert \mathcal{S} \rvert}\right)}^2\;,& \alpha=1 \;,
       \end{cases}
     \end{equation*}
     where $\mathcal{T}\subset\mathcal{S}$ denotes the set all strata
     that contain $\Gamma$.      
\end{lemma}
%
\begin{proof}
  For a uniform stratification we have
  $p_S = 1/\lvert \mathcal{S}\rvert$ for all $S\in\mathcal{S}$, so
  that the stratification estimator's variance can be written as
  \begin{equation*}
    \var{\hat{Q}_{\alpha}}  
    =\frac{ \Vert \boldsymbol{\sigma} \Vert_1}{N\, \lvert \mathcal{S}\rvert} \sum_{S\in\mathcal{S}}\frac{\sigma_S^2}{ \Vert \boldsymbol{\sigma} \Vert_1 + \alpha\left(\sigma_S \lvert \mathcal{S}\rvert - \Vert \boldsymbol{\sigma} \Vert_1 \right)}
    = \frac{ \Vert \boldsymbol{\sigma} \Vert_1}{N\, \lvert \mathcal{S}\rvert} \sum_{S\in\mathcal{S}}\frac{\sigma_S^2}{ (1-\alpha) \Vert \boldsymbol{\sigma} \Vert_1 + \alpha\sigma_S \lvert \mathcal{S}\rvert }\;.
  \end{equation*}
  %
  We proceed by bounding the local variances $\sigma_S^2$ in each
stratum $S\in\mathcal{S}$. To do this we distinguish the two
cases for the regularity of the function
$f\colon\mathfrak{U}\to\mathbb{R}$.

We begin with the case $f\in C^1(\mathfrak{U})$. It follows
from a Taylor expansion of $f$ and the Cauchy--Schwarz inequality that
\begin{equation*}
\sigma_S^2 = \var{Q_S} = \var{f(\bY)| \bY\in S} \le \sup_{\bu\in\mathfrak{U}} \Vert \nabla f(\bu) \Vert_{2}^2 \, \E{\Vert \bY \Vert_{2}^2} {\lvert \mathcal{S} \rvert}^{-2/n}    \;.
\end{equation*}
Noting that $\E{\Vert \bY \Vert_{2}^2} = n/3$, we obtain the bound
$\sigma_S^2 \le n\,C\, 3^{-1} {\lvert \mathcal{S} \rvert}^{-2/n}$ for
all $S\in\mathcal{S}$, where
$C = \sup_{\bu\in\mathfrak{U}} \Vert \nabla f(\bu) \Vert_{2}^2$.  We
thus have
$\Vert \boldsymbol{\sigma} \Vert_1^2 \le \frac{n\, C}{3}\, {\lvert
  \mathcal{S} \rvert}^{2-2/n}$.  Consequently, for $\alpha\in\{0,1\}$ the
estimator's variance satisfies
\begin{equation*}
    \var{\hat{Q}_{0}}  
    = \frac{ 1}{N\, \lvert \mathcal{S}\rvert} \sum_{S\in\mathcal{S}}\sigma_S^2 \le \frac{ n\, C}{\,3\,N} {\lvert \mathcal{S} \rvert}^{-2/n}\quad\text{and}\quad
    \var{\hat{Q}_{1}}  
    = \frac{ \Vert \boldsymbol{\sigma} \Vert_1^2}{N\, {\lvert \mathcal{S}\rvert}^2} \le \frac{n\, C}{3\, N}\,{\lvert \mathcal{S} \rvert}^{-2/n}\;,
  \end{equation*}
  respectively.  For the intermediate values $0< \alpha<1$ we use 
  \begin{equation*}
    (1-\alpha) \Vert \boldsymbol{\sigma} \Vert_1 + \alpha\sigma_S \lvert \mathcal{S}\rvert \ge
    \begin{cases}
      (1-\alpha) \Vert \boldsymbol{\sigma} \Vert_1\;,\\
      \alpha\sigma_S \lvert \mathcal{S}\rvert\;,
    \end{cases}
  \end{equation*}
which implies that {\color{blue} [mention earlier, when introducing hybrid? but then for non-uniform? what is the insight though, as it may not be sharp?]}
  \begin{equation}\label{eq:asymp:varred:hybird:bnd}
    \var{\hat{Q}_{\alpha}}  \le \begin{cases}
      \frac{1}{1-\alpha} \var{\hat{Q}_{0}}\;,\\
      \frac{1}{\alpha} \var{\hat{Q}_{1}}\;,
    \end{cases}
  \end{equation}
  for any $0< \alpha<1$. Using the established variance bound for the
  terms on the right hand sides and considering the minimum over both
  cases completes the proof.
  
  Next we consider the case of $f\colon \mathfrak{U}\to\mathbb{R}$
  being a piecewise constant function. In that case we have
  $\sigma_S^2 = 0$ for all
  $S\in\mathcal{S}\setminus\mathcal{T}$. Conversely, for
  $S\in\mathcal{T}$ the quantity $Q_S$ is a random variable taking two
  values probabilities proportional to the sizes of stratum
  subdivisions by $\Gamma$.  Consequently, $\sigma_S^2 \le \delta^2/4$,
  where $\delta>0$ is the height of the jump discontinuity. For
  $\alpha\in\{0,1\}$ the estimator's variance satisfies
\begin{equation*}
    \var{\hat{Q}_{0}}  
    = \frac{ 1}{N\, \lvert \mathcal{S}\rvert} \sum_{S\in\mathcal{S}}\sigma_S^2 \le \frac{\delta^2 {\lvert \mathcal{T}\rvert} }{4\,N\, {\lvert \mathcal{S}\rvert} }\quad\text{and}\quad
    \var{\hat{Q}_{1}}  
    = \frac{ \Vert \boldsymbol{\sigma} \Vert_1^2}{N\, {\lvert \mathcal{S}\rvert}^2} \le \frac{\delta^2 {\lvert \mathcal{T}\rvert}^2 }{4\,N\, {\lvert \mathcal{S}\rvert}^2} \;,
  \end{equation*}
  respectively, and from \eqref{eq:asymp:varred:hybird:bnd} we conclude that 
  \begin{equation*}
    \var{\hat{Q}_{\alpha}}  \le \frac{\delta^2 }{4\,N} \,\frac{{\lvert \mathcal{T}\rvert}} {\lvert \mathcal{S}\rvert}
    \min\left\{\frac{1}{1-\alpha}, \frac{1}{\alpha}\, \frac{\lvert \mathcal{T}\rvert}{\lvert \mathcal{S}\rvert}\right\}
  \end{equation*}
for any $0< \alpha<1$.  
    \end{proof}  

   Notice that the preceding lemma states that at last asymptotically,
   optimal allocation not superior to proportional allocation for
   smooth problems.

   {\color{blue} quasi-optimal for $\alpha \ge \gamma > \frac{\gamma}{\gamma+1}$ where $\gamma = \frac{\lvert \mathcal{T}\rvert}{\lvert \mathcal{S}\rvert}<1$.}



   \emph{quasi-optimal} sample allocation for $\alpha\in(0,1]$
   sufficiently large, but not only for $\alpha=1$.
   
   Example: $\mathcal{S} = K^n$, $\mathcal{T} = K^{n-1}$.
   \begin{enumerate}
   \item $f\in C^1(\mathfrak{U})$:
    \begin{equation*}
      \var{\hat{Q}_{\alpha}} \le \frac{n C}{3\, N}
         \min\left(\frac{1}{\alpha}, \frac{1}{1-\alpha}\right)\, {K}^{-2}\;,
     \end{equation*}
   \item $f\colon \mathfrak{U}\to\mathbb{R}$ is a piecewise
     constant
     \begin{equation*}
       \var{\hat{Q}_{\alpha}} \le \frac{\delta^2}{4\,N}
       \begin{cases}
         K^{-1}\;,& \alpha = 0\;,\\
         K{-1}\, \min\left\{\frac{1}{1-\alpha}, \frac{K^{-1}}{\alpha}\right\}\;,& 0<\alpha < 1 \;,\\
         K^{-2}\;,& \alpha=1 \;,
       \end{cases}
     \end{equation*}
     That is, for $\alpha> K^{-1}/(K^{-1}+1)$, e.g., $\alpha>K^{-1}$,
     we get \emph{quasi-optimal}
      variance reduction $\var{\hat{Q}_{\alpha}}\le \frac{\delta^2}{4\,\alpha \,N}\,
     K^{-2}$
   \end{enumerate}




   
   \begin{figure}
        \centering
        \includegraphics[width=0.25\textwidth]{../presentation/figs_strat_basics/discont_uniform}\quad
        \includegraphics[width=0.25\textwidth]{../presentation/figs_strat_basics/discont_adaptive}
        \caption{hello}
      \end{figure}

   


summary: robust and sub-optimal vs.\ volatile and optimal

% {\color{gray}
% That is, let
% $\theta\ge0$, then the probability of misestimating the true standard
% deviation by $\theta$ is
% \begin{equation}\label{eq:failure:prob:global:abs}
%   \begin{aligned}
%     \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
%     &=  \mathbb{P}\Bigl(\Bigl\vert \sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S) \Bigr\vert \ge \theta \sqrt{N}\Bigr)\\
%     &= \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S)  \ge \theta \sqrt{N}\Bigr) +
%     \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S)  \le -\theta \sqrt{N}\Bigr)\\
%     & =: P_1 + P_2\;.
%   \end{aligned}
% \end{equation}
% It follows from Markov's inequality that $P_1$ and $P_2$ can be bounded by 
% \begin{equation*}
%   P_1 \le e^{-t\theta\sqrt{N} }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{t(\hat\sigma_S - \sigma_S)p_S}\bigr)\;,\quad\text{and}\quad
%   P_2 \le e^{-t\theta\sqrt{N} }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{-t(\hat\sigma_S - \sigma_S)p_S}\bigr)\;,
% \end{equation*}
% respectively, for any $t>0$, where we have used the fact that
% $\hat\sigma_{S_1}$ and $\hat\sigma_{S_2}$ are independent for strata
% $S_1, S_2\in\mathcal{S}$ if $S_1\not= S_2$. Putting both estimates
% together and minimizing over $t>0$, we find the upper bound for the
% failure probability as
% \begin{equation}
%   \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
%   \le \min_{t>0}e^{-t\theta\sqrt{N} }\left(\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{t(\hat\sigma_S - \sigma_S)p_S}\bigr) + \prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{-t(\hat\sigma_S - \sigma_S)p_S}\bigr)\right)\;.\label{eq:failure:prob:global:hoeffding:abs}
% \end{equation}
% For certain functions $f$ it may be possible to deduce the
% distribution of $Y_S := f(\boldsymbol{Z}_S)$, and thus also of
% $\hat\sigma_S = \sqrt{h_2(S)}$,\footnote{Or making a Gaussian
%   approximation...} which may allow to compute the moment generating
% function $\tau\mapsto \mathbb{E}(e^{\tau\hat\sigma_S})$ in closed
% form. However, this does not seem to be the case in general. On the
% other hand, if $0\le \hat\sigma_S$ is almost surely bounded, then we
% can use Hoeffding's lemma to derive more insightful estimates. Indeed,
% such a boundedness assumption seems reasonable, in particular when
% assuming that $f$ does not contain any singularities in $S$. In fact,
% if $-\infty< l_S := \inf_S f \le \sup_S f =: u_S <\infty$, then
% $h_2(S) \le \frac{N}{N-1}({u_S}^2 - {l_S}^2) \le 2({u_S}^2 - {l_S}^2)
% $. We thus suppose that $0\le m_S\le \hat\sigma_S\le M_S$ almost
% surely on stratum $S$. In view of Hoeffding's lemma we then find
% \begin{equation*}
%   \prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{\pm t(\hat\sigma_S - \sigma_S)p_S}\bigr) \le \prod_{S\in\mathcal{S}} e^{\pm tp_S\delta(S) + t^2 {p_S}^2 \frac{{(M_S - m_S)}^2}{8}}
%   = e^{\pm t\sum_{S\in\mathcal{S}} p_S \delta(S) + \frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\;,
% \end{equation*}
% where $\delta(S) := \mathbb{E}(\hat\sigma_S) - \sigma_S$ denotes the
% bias of the empirical standard deviation estimator
% $\hat\sigma_S = \sqrt{h_2(S)}$. Notice that $\delta(S)$ is not zero,
% despite the fact that $\hat\sigma_S^2 \equiv h_2(S)$ is an unbiased
% estimator of $\mu_2(S) \equiv \sigma_S^2$ due to the non-linearity of
% the square root. In fact, it is known that
% $\delta(S)= \mathcal{O}(1/N_S)$ and, moreover, that one cannot find an
% empirical standard deviation estimator that is unbiased for all
% distributions. Using the upper bound in
% \eqref{eq:failure:prob:global:hoeffding:abs}, we eventually obtain
% \begin{equation}\label{eq:failure:prob:global:hoeffding:abs:final}
%   \begin{aligned}
%     \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
%     &\le \min_{t>0} e^{-t\theta\sqrt{N} + \frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2} \Bigl( e^{ t\sum_{S\in\mathcal{S}} p_S \delta(S)}
%     + e^{-t\sum_{S\in\mathcal{S}} p_S \delta(S)}\Bigr)\\
%     & \le 2 \min_{t>0} e^{\frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2 + t\left(\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert - \theta\sqrt{N}\right)}\\
%     & = 2 \exp{\left(-\frac{2{\left(\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert - \theta\sqrt{N}\right)}^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;,
%   \end{aligned}
% \end{equation}
% provided that
% \begin{equation*}
%   \theta > \frac{1}{\sqrt{N}} \sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert\;.
% \end{equation*}
% Notice that the bound
% \eqref{eq:failure:prob:global:hoeffding:abs:final} also offers an
% estimate for the relative error, which provides insight into the
% effect of the given stratification alone. To see this, set
% $R := \sqrt{\hat{V}/\mathcal{V}}$ and use
% $\theta = \tau \sqrt{\mathcal{V}} \equiv \tau
% \varsigma/\sqrt{N}$ for a suitable $\tau\ge 0$, where
% $\varsigma := \sum_{S\in\mathcal{S}}p_S \sigma_S$. Then
% \eqref{eq:failure:prob:global:hoeffding:abs:final} can be restated as
% \begin{equation}\label{eq:failure:prob:global:hoeffding:rel:final}
%     \mathbb{P}\bigl(\lvert R - 1 \rvert \ge \tau \bigr)
%     \le 2 \exp{\left(-\frac{2{\left(\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert - \tau\varsigma\right)}^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;,
% \end{equation}
% provided that
% \begin{equation*}
%   \tau > \frac{\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert}{\varsigma}
%   = \frac{\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert}{\sum_{S\in\mathcal{S}} p_S\sigma_S}\;.
% \end{equation*}

% }




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Master"
%%% End:

==> failure_probs.tex <==
% \section{Probability of failure to identify a stratum that should be split}
% {\color{red}[Replace $\boldsymbol{X}$ with $\boldsymbol{Y}$ below, for consistency with previous notation?]}
% The adaptive method's increased variance reduction is achieved by
% splitting strata with high variances (more precisely, splitting those
% for which the product of variance and measure is large). That is, it
% relies on informative variance estimators of $Y = f(\boldsymbol{X})$ conditional
% upon $\boldsymbol{X}\in S$ for every stratum $S$. For a given stratum $S$, let
% $\mu_2\equiv\mu_2(Y)$ denote the variance (central moment of order
% $2$) of $Y$ conditional upon $\boldsymbol{X}\in S$ and denote by $h_2\equiv h_2(Y)$
% the corresponding unbiased sample variance estimator (h-statistics of
% order 2) based on $M$ samples. Observe that $\mu_2=0$ implies that
% $h_2 = 0$ and, conversely, that $h_2>0$ implies $\mu_2>0$.

% The method's efficiency may deteriorate if the sample variance is
% drastically underestimating the true variance. This can happen for
% example, if the stratum does not contain enough samples, so that a
% discontinuity is not observed given these samples. In view of the
% implications mentioned above, this can only occur if $\mu_2>0$. To
% further quantify this ``failure'', suppose there that $\mu_2>0$. As
% $h_2\ge 0$, it follows from the Paley--Zygmund inequality (combined
% with the Cauchy--Schwarz inequality) that
% \begin{equation*}
%   \mathbb{P}(h_2 > \theta \mu_2) \ge \frac{(1-\theta)^2 {\mu_2}^2}{(1-\theta)^2 {\mu_2}^2 + \var{h_2}}
%   = \frac{(1-\theta)^2 {\mu_2}^2}{(1-\theta)^2 {\mu_2}^2 + M^{-1}\left( \mu_4 - \frac{M-3}{M-1}{\mu_2}^2\right)}\;,
% \end{equation*}
% for any $\theta\in [0,1]$. Let $\kappa := \frac{\mu_4}{{\mu_2}^2}$
% denote the kurtosis of $Y$, given $\boldsymbol{X}\in S$. Then it follows that
% \begin{equation}
%   \mathbb{P}(h_2 \le \theta \mu_2) \le 1-  \frac{(1-\theta)^2}{(1-\theta)^2 + M^{-1}\left( \kappa - \frac{M-3}{M-1}\right)} =
%   \frac{\kappa - \frac{M-3}{M-1}}{M (1-\theta)^2 + \left( \kappa - \frac{M-3}{M-1}\right)}\;.\label{eq:failure:prob}
% \end{equation}
% The preceding inequality indicates that the probability of
% underestimating the variance of $Y = f(\boldsymbol{X})$ given that $\boldsymbol{X}\in S$ by a
% factor $\theta$ is of order $\mathcal{O}(1/M)$. In fact, if $\kappa$
% was known, one could use the upper bound to determine the required
% sample size $M$ to guaranteed that
% $\mathbb{P}(h_2 \le \theta \mu_2)\le p_{\text{crit}}$ for some
% tolerance $p_{\text{crit}} \in(0,1)$.  However, the upper bound also
% reveals that it is strongly affected by the kurtosis $\kappa$, in the
% sense that a higher kurtosis leads to a higher probability of
% underestimating the variance:
% \begin{equation*}
%   \mathbb{P}(h_2 \le \theta \mu_2) \le 
%   \frac{\kappa - \frac{M-3}{M-1}}{M (1-\theta)^2 + \left( \kappa - \frac{M-3}{M-1}\right)} = \frac{\kappa-1}{M(1-\theta)^2} + \mathcal{O}(M^{-2})\;.
% \end{equation*}
% %
% Although the kurtosis $\kappa$ is well-known for many distributions,
% it remains to address how this upper bound could be used in practice
% where it is usually not known.  In the context of the proposed
% stratified sampling procedure, an exemplary borderline case is when
% the stratum $S$ contains a region $R\subset S$,
% $S\setminus R \not=\emptyset$, on which $f$ is constant and all
% available samples are contained in $R$. That is,
% $\boldsymbol{X}^{(1)},\dots, \boldsymbol{X}^{(M)} \in R$ so that $Y_i = f(\boldsymbol{X}^{(i)}) \equiv f_R$ for all
% $i=1,\dots, M$. It follows that $h_2=0$ in that case, despite the fact that
% $\mu_2>0$, since not the entire stratum has been sampled from and the
% region $S\setminus R$ has been missed. Consequently, this can lead to
% a ``failure'' of the adaptive procedure, in the sense that splitting a
% high variance stratum may be missed, resulting in a sub-optimal
% performance. Moreover, the bound on the failure probability in
% \eqref{eq:failure:prob} is also not of any help in that case, unless
% we know the true kurtosis $\kappa$. In fact, estimating the kurtosis
% by the ratio of $h_2$ and $h_4$ (the fourth order $h$-statistic) will
% be undefined in that case.  A possible remedy would be in use a
% rule-of-thumb, such as assuming that $Y$ follows a normal distribution
% ($\kappa=3$), a uniform distribution on some interval
% ($\kappa = 9/5$), or some other distribution with known kurtosis; see
% Fig.~\ref{fig:failure:prob:examples} for examples of the upper bound
% on the failure probability in \eqref{eq:failure:prob} for two
% different distributions.
% \begin{figure}[tb!]
%   \centering
%   \includegraphics[width=0.4\textwidth]{./figures/GaussianFailureProb}\quad
%   \includegraphics[width=0.4\textwidth]{./figures/UniformFailureProb}
%   \caption{Upper bound failure probability for a Gaussian distribution (left) and a uniform distribution (right).}
%   \label{fig:failure:prob:examples}
% \end{figure}
% Recall that theses upper bounds quantify the failure probability
% conditional upon $\boldsymbol{X}\in S$ and not the entire method's failure
% probability.

% \subsection{KDE-based estimation}
% Alternatively, a data-driven (i.e., sample based) approach using KDE
% moment approximations will always be possible. In fact, even in the
% borderline case when obtaining only samples from the region $R$ where
% $f$ is constant, this KDE approach, interestingly, yields a Gaussian
% kurtosis rule-of-thumb approximation as we will see below.
% %
% % To see this, recall $\mu_2>0$
% % but $h_2=0$ in that case, since not the entire stratum has been
% % sampled.
% In general, the KDE-based moments are given by
% \[
% m_{k,\scriptscriptstyle{\textup{KDE}}}(Y) = \frac{1}{n} \sum_{i=1}^{M}\int y^k K_\delta(y-Y_i)\,dy\;,
% \]
% which yields
% \begin{equation}
% \begin{aligned}
% m_{1,\scriptscriptstyle{\textup{KDE}}}(Y) &= \frac{1}{M} \sum_{i=1}^{M}Y_{i}\;, \\ %\notag \\
% m_{2,\scriptscriptstyle{\textup{KDE}}}(Y) &= \frac{1}{M} \sum_{i=1}^{M}Y_{i}^2 + \delta^2, \\ %  \notag \\
% m_{3,\scriptscriptstyle{\textup{KDE}}}(Y) &= \frac{1}{M}\sum_{i=1}^{M}Y_{i}^{3} + 3\delta^2\frac{1}{M}\sum_{i=1}^{M}Y_{i}, \\%\notag \\
% m_{4,\scriptscriptstyle{\textup{KDE}}}(Y) &= \frac{1}{M}\sum_{i=1}^{M}Y_{i}^{4} + 6\delta^2 \frac{1}{M}\sum_{i=1}^{M}Y_{i}^2  + 3\delta^4\;.%\notag
% \end{aligned}
% \label{eq:KDE_moments}
% \end{equation}
% Except for the first moment, the KDE moments differ by a term
% $\mathcal{O}(\delta^2)$ from the empirical moments computed directly from
% data, which can be viewed as a smoothing. Consequently, the approximation
% \begin{equation*}
%   \kappa \approx \hat\kappa := \frac{m_{4,\scriptscriptstyle{\textup{KDE}}}(Y) - 4m_{1,\scriptscriptstyle{\textup{KDE}}}(Y) m_{3,\scriptscriptstyle{\textup{KDE}}}(Y) + 6 m_{1,\scriptscriptstyle{\textup{KDE}}}(Y)^2m_{2,\scriptscriptstyle{\textup{KDE}}}(Y) - 3 m_{1,\scriptscriptstyle{\textup{KDE}}}(Y)^4}{{\left(m_{2,\scriptscriptstyle{\textup{KDE}}}(Y) - m_{1,\scriptscriptstyle{\textup{KDE}}}(Y)^2\right)}^2}
% \end{equation*}
% is always well-defined. In fact, even in the borderline case with
% $Y_1 = Y_2 = \dots Y_M = f_R$. Then we find
% \begin{equation*}
%   \begin{aligned}
%   m_{1,\scriptscriptstyle{\textup{KDE}}}(Y) &= Y_1\;,\quad m_{2,\scriptscriptstyle{\textup{KDE}}}(Y) = {Y_1}^2 + \delta^2\;,\\
%   m_{3,\scriptscriptstyle{\textup{KDE}}}(Y) &= {Y_1}^3 + 3\delta^2Y_1\;, \quad m_{4,\scriptscriptstyle{\textup{KDE}}}(Y) = {Y_1}^4 + 6\delta^2 {Y_1}^2 + 3\delta^4\;,
% \end{aligned}
% \end{equation*}
% which yields
% \begin{equation*}
%   \hat\kappa = \frac{{Y_1}^4 + 6\delta^2 {Y_1}^2 + 3\delta^4 - 4\left({Y_1}^4 + 3\delta^2{Y_1}^2 \right) + 6\left({Y_1}^4 + {Y_1}^2\delta^2 \right)- 3{Y_1}^4}{{\left({Y_1}^2 + \delta^2 - {Y_1}^2\right)}^2} = 3\;.
% \end{equation*}
% That is, the KDE-based moment approximation corresponds to the
% Gaussian rule of thumb, for any bandwidth parameter $\delta$.


\section{\sout{Probability of failure: an a-posteriori point of view}} {\color{gray}\textbf{remove entirely?}
% While the previous subsection addressed the failure to identify a high
% variance region, the main goal in practice is to quantify the
% performance of the adaptive stratification estimator. Recall that the
% adaption is motivated to maintain an effective variance reduction even
% in the presence of heterogeneous features. That is, the adaptive
% iterative procedure outlined above yields, roughly
% speaking,\footnote{Actually, I think it will not possible to make this
%   really exact, as we will have dependencies on the previously sampled
%   variables. To overcome this, one could use $N/2$ samples to learn
%   the stratification. Then fix the obtained stratification and use the
%   remaining $N/2$ as in usual stratification estimator. However, to be
%   fair, we will then have to compare the variance reduction of our
%   method using $N/2$ samples with Monte Carlo using N samples. } a
% stratification of the sampling domain, so that the estimator at the
% final iteration can be viewed a classic stratification estimator. The
% crucial difference is, of course, that its stratification has been
% adapted to the problem at hand.  Nonetheless, given a stratification,
% the theoretical results available for classic stratification
% estimators apply here; see. e.g., \cite[Ch.~V,
% Sect.~7]{Asmussen_Glynn_07}. To be more precise, recall that the
% stratification estimator $\hat{f}_{\text{strat}}$ of
% $\mathbb{E}\bigl(f(\boldsymbol{X})\bigr)$ is
% \begin{equation*}
%   \hat{f}_{\text{strat}} := \sum_{S\in\mathcal{S}}p_SE_{N_S}^{\text{mc}}\bigl(f(\boldsymbol{X}) \bigl.\bigr\vert \boldsymbol{X}\in S\bigr) \equiv \sum_{S\in\mathcal{S}}\frac{p_S}{N_S} \sum_{i=1}^{N_S}f\bigl(\boldsymbol{Z}_S^{(i)}\bigr)\;,
% \end{equation*}
% for a given stratification $\mathcal{S}$, where $\boldsymbol{Z}_S$ is
% distributed according to the conditional distribution of
% $\boldsymbol{X}$ given that $\boldsymbol{X}\in S$. Moreover, let
% $N:= \sum_{S\in\mathcal{S}} N_S$ denote the total number of
% samples. For a given stratification $\mathcal{S}$ the estimator
% $\hat{f}_{\text{strat}}$ is unbiased
% \begin{equation*}
%   \mathbb{E}\bigl( \hat{f}_{\text{strat}} \bigr) = \sum_{S\in\mathcal{S}}\mathbb{P}(\boldsymbol{X}\in S) \mathbb{E}\bigl(f(\boldsymbol{X}) \bigl.\bigr\vert \boldsymbol{X}\in S\bigr) = \mathbb{E}\bigl( f(\boldsymbol{X})\bigr)
% \end{equation*}
% and its variance is given by
% \begin{equation*}
%   \var{\hat{f}_{\text{strat}} } = \sum_{S\in\mathcal{S}}{\mathbb{P}(\boldsymbol{X}\in S)}^2 \frac{\var{f(\boldsymbol{X}) \bigl.\bigr\vert \boldsymbol{X}\in S}}{N_S} = \sum_{S\in\mathcal{S}}{\mathbb{P}(\boldsymbol{X}\in S)}^2 \frac{\var{f(\boldsymbol{Z}_S)}}{N_S}
% \end{equation*}
% for any number of samples per strata $N_S$,
% $S\in\mathcal{S}$. Moreover, if $N_S$ is such that
% $\lim_{N\to\infty}\frac{N}{N_S} < \infty$, then
% $\lim_{N\to\infty} N \var{\hat{f}_{\text{strat}} } < \infty$ and
% $\hat{f}_{\text{strat}}$ satisfies the central limit theorem
% \begin{equation*}
%   \frac{\hat{f}_{\text{strat}} - \mathbb{E}\bigl( f(\boldsymbol{X})\bigr) }{\sqrt{\var{\hat{f}_{\text{strat}} }} } \underset{N\to\infty}{\Rightarrow}\mathcal{N}(0,1)\;.
% \end{equation*}
% In practice when $N\gg 1$, this asymptotic normality can thus be used
% to not only report a point estimate for
% $\mathbb{E}\bigl( f(\boldsymbol{X})\bigr)$ (i.e., simply the obtained
% value $\hat{f}_{\text{strat}}$), also an approximate confidence
% region. For example, let $q_{1-\alpha/2}$ be the $1-\alpha/2$ quantile
% of the standard normal distribution so that 
% \begin{equation*}
%   \begin{aligned}
%     1-\alpha &\approx \mathbb{P}\left( {\var{\hat{f}_{\text{strat}} }}^{-1/2}\left\vert \hat{f}_{\text{strat}} - \mathbb{E}\bigl( f(\boldsymbol{X})\bigr) \right\vert \le q_{1-\alpha/2}\right)\\
%     &= \mathbb{P}\left( \hat{f}_{\text{strat}} -  q_{1-\alpha/2} \sqrt{\var{\hat{f}_{\text{strat}} }} \le \mathbb{E}\bigl( f(\boldsymbol{X})\bigr) \le  \hat{f}_{\text{strat}} +  q_{1-\alpha/2} \sqrt{\var{\hat{f}_{\text{strat}} }}\right)\;.
%   \end{aligned}
%   \end{equation*}
%   In other words: the unknown value
%   $\mathbb{E}\bigl( f(\boldsymbol{X})\bigr)$ is contained in the
%   confidence interval
%   \begin{equation*}
%     I_{\alpha} := \left[ \hat{f}_{\text{strat}} -  q_{1-\alpha/2}\sqrt{\var{\hat{f}_{\text{strat}} }}  , \hat{f}_{\text{strat}} +  q_{1-\alpha/2}  \sqrt{\var{\hat{f}_{\text{strat}} }}\right]
%   \end{equation*}
%   with probability approximately equal to $1-\alpha$.
% %
%   An alternative approach to quantifying the probability of failure is,
%   of course, in view of Chebyshev's inequality:
%   \begin{equation*}
%     \mathbb{P} \Bigl(\bigl\vert\hat{f}_{\text{strat}} - \mathbb{E}\bigl( f(\boldsymbol{X})\bigr) \bigr\vert \ge \theta \Bigr) \le \frac{\var{\hat{f}_{\text{strat}} }}{\theta^2}\;,
%   \end{equation*}
%   for any $\theta>0$. While this estimate does not rely on an
%   asymptotic normality assumption, it may be not as sharp as the
%   corresponding statement based on a normal approximation if $N\gg 1$.

%   What both estimates have in common is that they are controlled by
%   the estimator's variance. However, for these approaches to be
%   practical, we require an accurate estimation of the stratification
%   estimator's standard deviation or variance. Next, we will quantify
%   the probability of misestimating the standard
%   deviation. {\color{green} maybe the following was useless and we
%     should have done var directly, which seems more tedious though?}

% \subsubsection{Quantifying the accuracy of the variance estimators}

% Notice that the consideration above are independent of the sample
% allocation rule.\footnote{This got me thinking: is there a benefit
%   from using the sub-optimal proportional sample allocation rule while
%   learning the problem adapted stratification? At first glance I thought
%   so, since the rule does not require variance estimates. However,
%   that is an incomplete reasoning, because we need the variance for
%   the splitting any ways, so one can also use this during the sample
%   allocation rule, right? Do you think it makes sense to do numerics
%   comparing both?}  Using an optimal sample allocation per stratum,
% that is
% $N_S = \frac{p_S\sigma_S}{\sum_{S\in \mathcal{S}}p_S \sigma_S} N$ with
% $\sigma_S \equiv \sqrt{\mu_2(S)} := \sqrt{\var{f(\boldsymbol{Z}_S)}}$
% denoting the conditional (output) standard deviation in stratum $S$,
% the stratification estimator's variance is
% \begin{equation*}
%   \mathcal{V} := \var{\hat{f}_{\text{strat}}} = \frac{1}{N} {\Bigl(\sum_{S\in\mathcal{S}}p_S \sigma_S\Bigr)}^2\;.
% \end{equation*}
% Given a
% stratification, the natural variance estimate thus is
% \begin{equation*}
%   \hat{V} := \frac{1}{N} {\Bigl(\sum_{S\in\mathcal{S}}p_S \hat{\sigma}_S\Bigr)}^2\;,
% \end{equation*}
% where $\hat{\sigma}_S := \sqrt{h_2(S)}$ denotes standard empirical
% standard deviation based on $N_S$ samples in stratum $S$. Based on
% this variance estimate, we can then quantify the probability of
% failure, in the sense of a variance misestimation. That is, let
% $\theta\ge0$, then the probability of misestimating the true standard
% deviation by $\theta$ is
% \begin{equation}\label{eq:failure:prob:global:abs}
%   \begin{aligned}
%     \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
%     &=  \mathbb{P}\Bigl(\Bigl\vert \sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S) \Bigr\vert \ge \theta \sqrt{N}\Bigr)\\
%     &= \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S)  \ge \theta \sqrt{N}\Bigr) +
%     \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S)  \le -\theta \sqrt{N}\Bigr)\\
%     & =: P_1 + P_2\;.
%   \end{aligned}
% \end{equation}
% It follows from Markov's inequality that $P_1$ and $P_2$ can be bounded by 
% \begin{equation*}
%   P_1 \le e^{-t\theta\sqrt{N} }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{t(\hat\sigma_S - \sigma_S)p_S}\bigr)\;,\quad\text{and}\quad
%   P_2 \le e^{-t\theta\sqrt{N} }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{-t(\hat\sigma_S - \sigma_S)p_S}\bigr)\;,
% \end{equation*}
% respectively, for any $t>0$, where we have used the fact that
% $\hat\sigma_{S_1}$ and $\hat\sigma_{S_2}$ are independent for strata
% $S_1, S_2\in\mathcal{S}$ if $S_1\not= S_2$. Putting both estimates
% together and minimizing over $t>0$, we find the upper bound for the
% failure probability as
% \begin{equation}
%   \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
%   \le \min_{t>0}e^{-t\theta\sqrt{N} }\left(\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{t(\hat\sigma_S - \sigma_S)p_S}\bigr) + \prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{-t(\hat\sigma_S - \sigma_S)p_S}\bigr)\right)\;.\label{eq:failure:prob:global:hoeffding:abs}
% \end{equation}
% For certain functions $f$ it may be possible to deduce the
% distribution of $Y_S := f(\boldsymbol{Z}_S)$, and thus also of
% $\hat\sigma_S = \sqrt{h_2(S)}$,\footnote{Or making a Gaussian
%   approximation...} which may allow to compute the moment generating
% function $\tau\mapsto \mathbb{E}(e^{\tau\hat\sigma_S})$ in closed
% form. However, this does not seem to be the case in general. On the
% other hand, if $0\le \hat\sigma_S$ is almost surely bounded, then we
% can use Hoeffding's lemma to derive more insightful estimates. Indeed,
% such a boundedness assumption seems reasonable, in particular when
% assuming that $f$ does not contain any singularities in $S$. In fact,
% if $-\infty< l_S := \inf_S f \le \sup_S f =: u_S <\infty$, then
% $h_2(S) \le \frac{N}{N-1}({u_S}^2 - {l_S}^2) \le 2({u_S}^2 - {l_S}^2)
% $. We thus suppose that $0\le m_S\le \hat\sigma_S\le M_S$ almost
% surely on stratum $S$. In view of Hoeffding's lemma we then find
% \begin{equation*}
%   \prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{\pm t(\hat\sigma_S - \sigma_S)p_S}\bigr) \le \prod_{S\in\mathcal{S}} e^{\pm tp_S\delta(S) + t^2 {p_S}^2 \frac{{(M_S - m_S)}^2}{8}}
%   = e^{\pm t\sum_{S\in\mathcal{S}} p_S \delta(S) + \frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\;,
% \end{equation*}
% where $\delta(S) := \mathbb{E}(\hat\sigma_S) - \sigma_S$ denotes the
% bias of the empirical standard deviation estimator
% $\hat\sigma_S = \sqrt{h_2(S)}$. Notice that $\delta(S)$ is not zero,
% despite the fact that $\hat\sigma_S^2 \equiv h_2(S)$ is an unbiased
% estimator of $\mu_2(S) \equiv \sigma_S^2$ due to the non-linearity of
% the square root. In fact, it is known that
% $\delta(S)= \mathcal{O}(1/N_S)$ and, moreover, that one cannot find an
% empirical standard deviation estimator that is unbiased for all
% distributions. Using the upper bound in
% \eqref{eq:failure:prob:global:hoeffding:abs}, we eventually obtain
% \begin{equation}\label{eq:failure:prob:global:hoeffding:abs:final}
%   \begin{aligned}
%     \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
%     &\le \min_{t>0} e^{-t\theta\sqrt{N} + \frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2} \Bigl( e^{ t\sum_{S\in\mathcal{S}} p_S \delta(S)}
%     + e^{-t\sum_{S\in\mathcal{S}} p_S \delta(S)}\Bigr)\\
%     & \le 2 \min_{t>0} e^{\frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2 + t\left(\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert - \theta\sqrt{N}\right)}\\
%     & = 2 \exp{\left(-\frac{2{\left(\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert - \theta\sqrt{N}\right)}^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;,
%   \end{aligned}
% \end{equation}
% provided that
% \begin{equation*}
%   \theta > \frac{1}{\sqrt{N}} \sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert\;.
% \end{equation*}
% Notice that the bound
% \eqref{eq:failure:prob:global:hoeffding:abs:final} also offers an
% estimate for the relative error, which provides insight into the
% effect of the given stratification alone. To see this, set
% $R := \sqrt{\hat{V}/\mathcal{V}}$ and use
% $\theta = \tau \sqrt{\mathcal{V}} \equiv \tau
% \varsigma/\sqrt{N}$ for a suitable $\tau\ge 0$, where
% $\varsigma := \sum_{S\in\mathcal{S}}p_S \sigma_S$. Then
% \eqref{eq:failure:prob:global:hoeffding:abs:final} can be restated as
% \begin{equation}\label{eq:failure:prob:global:hoeffding:rel:final}
%     \mathbb{P}\bigl(\lvert R - 1 \rvert \ge \tau \bigr)
%     \le 2 \exp{\left(-\frac{2{\left(\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert - \tau\varsigma\right)}^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;,
% \end{equation}
% provided that
% \begin{equation*}
%   \tau > \frac{\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert}{\varsigma}
%   = \frac{\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert}{\sum_{S\in\mathcal{S}} p_S\sigma_S}\;.
% \end{equation*}




% %%%%%%%%%%%%%%%%%%%
% % previous version
% %%%%%%%%%%%%%%%%%%%
% % As the stratification estimate is designed to offer a variance
% % reduction, it seems natural to also quantify the method's ``failure'' in
% % terms of the ratio of estimated and exact variance. That is, we wish
% % to quantify the probability that $\hat{V}/\mathcal{V}$, or
% % equivalently $R := \sqrt{\hat{V}/\mathcal{V}}$, differs significantly from
% % $1$. Let $\tau>0$, then
% % \begin{equation}\label{eq:failure:prob:global:rel}
% %   \begin{aligned}
% %   \mathbb{P}\bigl(\lvert R - 1 \rvert \ge \tau \bigr)
% %   &= \mathbb{P}\bigl(\sum_{S\in\mathcal{S}}p_S (\hat{\sigma}_S -\sigma_S)\ge \tau \sum_{S\in\mathcal{S}}p_S {\sigma}_S\bigr) \\
% %   &\qquad +  \mathbb{P}\bigl(\sum_{S\in\mathcal{S}}p_S (\hat{\sigma}_S-\sigma_S) \le -\tau \sum_{S\in\mathcal{S}}p_S \sigma_S\bigr)\\
% %   & =: P_1 + P_2 \;.
% % \end{aligned}
% % \end{equation}
% % We use the Chernoff bound (or rather Markov inequality) to derive upper
% % bounds for both $P_1$ and $P_2$. Indeed, let
% % $\varsigma := \sum_{S\in\mathcal{S}}p_S \sigma_S$, then we find for
% % \begin{equation*}
% %   P_1 \le e^{-t\tau \varsigma }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{t(\hat\sigma_S - \sigma_S)p_S}\bigr)\;,\quad\text{and}\quad
% %   P_2 \le e^{-t\tau \varsigma }\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{-t(\hat\sigma_S - \sigma_S)p_S}\bigr)\;,
% % \end{equation*}
% % for any $t>0$, where we have used the fact that $\hat\sigma_{S_1}$ and
% % $\hat\sigma_{S_2}$ are independent for strata $S_1, S_2\in\mathcal{S}$
% % if $S_1\not= S_2$. Putting both estimates together and minimizing over
% % $t>0$, we find the upper bound for the failure probability as
% % \begin{equation}
% %   \mathbb{P}\bigl(\lvert R - 1 \rvert \ge \tau \bigr)
% %   \le \min_{t>0}e^{-t\tau \varsigma }\left(\prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{t(\hat\sigma_S - \sigma_S)p_S}\bigr) + \prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{-t(\hat\sigma_S - \sigma_S)p_S}\bigr)\right)\;.\label{eq:failure:prob:global:hoeffding}
% % \end{equation}
% % For certain functions $f$ it may be possible to deduce the
% % distribution of $Y_S := f(\boldsymbol{Z}_S)$, and thus also of
% % $\hat\sigma_S = \sqrt{h_2(S)}$,\footnote{Or making a Gaussian
% %   approximation...} which may allow to compute the moment generating
% % function $s\mapsto \mathbb{E}(e^{s\hat\sigma_S})$ in closed
% % form. However, this does not seem to be the case in general. On the
% % other hand, if $0\le \hat\sigma_S$ is almost surely bounded, then we
% % can use Hoeffding's lemma to derive more insightful estimates. Indeed,
% % such an boundedness assumption seems reasonable, in particular when
% % assuming that $f$ does not contain any singularities in $S$. In fact,
% % if $-\infty< l_S := \inf_S f \le \sup_S f =: u_S <\infty$, then
% % $h_2(S) \le \frac{N}{N-1}({u_S}^2 - {l_S}^2) \le 2({u_S}^2 - {l_S}^2)
% % $. We thus suppose that $0\le m_S\le \hat\sigma_S\le M_S$ almost
% % surely on stratum $S$. In view of Hoeffding's lemma we then find
% % \begin{equation*}
% %   \prod_{S\in\mathcal{S}}\mathbb{E}\bigl(e^{\pm t(\hat\sigma_S - \sigma_S)p_S}\bigr) \le \prod_{S\in\mathcal{S}} e^{\pm tp_S\delta(S) + t^2 {p_S}^2 \frac{{(M_S - m_S)}^2}{8}}
% %   = e^{\pm t\sum_{S\in\mathcal{S}} p_S \delta(S) + \frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\;,
% % \end{equation*}
% % where $\delta(S) := \mathbb{E}(\hat\sigma_S) - \sigma_S$ denotes the
% % bias of the empirical standard deviation estimator
% % $\hat\sigma_S = \sqrt{h_2(S)}$. Notice that $\delta(S)$ is not zero,
% % despite the fact that $\hat\sigma_S^2 \equiv h_2(S)$ is an unbiased
% % estimator of $\mu_2(S) \equiv \sigma_S^2$ due to the non-linearity of
% % the square root. In fact, it is known that
% % $\delta(S)= \mathcal{O}(1/N_S)$ and, moreover, that one cannot find an
% % empirical standard deviation estimator that is unbiased for all
% % distributions. Using the upper bound in
% % \eqref{eq:failure:prob:global:hoeffding}, we eventually obtain
% % \begin{equation}\label{eq:failure:prob:global:hoeffding:final}
% %   \begin{aligned}
% %     \mathbb{P}\bigl(\lvert R - 1 \rvert \ge \tau \bigr)
% %     &\le \min_{t>0} e^{-t\tau\varsigma + \frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2} \Bigl( e^{ t\sum_{S\in\mathcal{S}} p_S \delta(S)}
% %     + e^{-t\sum_{S\in\mathcal{S}} p_S \delta(S)}\Bigr)\\
% %     & \le 2 \min_{t>0} e^{\frac{t^2}{8}\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2 + t\left(\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert - \tau\varsigma\right)}\\
% %     & = 2 \exp{\left(-\frac{2{\left(\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert - \tau\varsigma\right)}^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;,
% %   \end{aligned}
% % \end{equation}
% % provided that
% % \begin{equation*}
% %   \tau > \frac{\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert}{\varsigma}
% %   = \frac{\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert}{\sum_{S\in\mathcal{S}} p_S\sigma_S}\;.
% % \end{equation*}
% % As $\delta(S) = \mathcal{O}(1/N_S)$, the condition on $\tau$ reduces
% % to $\tau>0$ asymptotically and
% % \begin{equation*}
% %   \mathbb{P}\bigl(\lvert R - 1 \rvert \ge \tau \bigr) \lesssim
% %   2 \exp{\left(-\frac{2\tau^2\varsigma^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;.
% % \end{equation*}

% {\color{gray}\textbf{Seb: remove the following?}\\
% Note that a related approach to quantifying a failure probability can
% be obtained by considering the probability that the estimator's
% estimated standard deviation significantly differs from the theoretical
% standard deviation. That is,
% \begin{equation}\label{eq:failure:prob:global2}
%   \begin{aligned}
%     \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
%     &=  \mathbb{P}\Bigl(\Bigl\vert \sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S) \Bigr\vert \ge \theta \sqrt{N}\Bigr)\\
%     &= \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S)  \ge \theta \sqrt{N}\Bigr) +
%     \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S(\hat\sigma_S - \sigma_S)  \le -\theta \sqrt{N}\Bigr)\\
%     & =: P_1 + P_2\;,
% \end{aligned}
% \end{equation}
% for some $\theta>0$.  Suppose, as before, that $f$ is such that
% $0\le m_S\le \hat\sigma_S\le M_S$ almost surely on stratum $S$. In
% view of Hoeffding's inequality we then find
% \begin{equation*}
%   \begin{aligned}
%     P_1 &= \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S\bigl(\hat\sigma_S - \mathbb{E}(\hat\sigma_S)\bigr)  \ge \theta \sqrt{N} - \sum_{S\in\mathcal{S}}p_S\delta(S)\Bigr)\\
%     &\le \exp{\left(-\frac{2N{\Bigl(\theta-\frac{1}{\sqrt{N}}\sum_{S\in\mathcal{S}}p_S\delta(S)\Bigr)}^2}{\sum_{S\in\mathcal{S}} {(M_S - m_S)}^2}\right)}
%   \end{aligned}
% \end{equation*}
% as well as
% \begin{equation*}
%   \begin{aligned}
%     P_2 &= \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S\bigl(\hat\sigma_S - \mathbb{E}(\hat\sigma_S)\bigr)  \le -\theta \sqrt{N} - \sum_{S\in\mathcal{S}}p_S\delta(S)\Bigr)\\
%     &= \mathbb{P}\Bigl(\sum_{S\in\mathcal{S}}p_S\bigl(\mathbb{E}(\hat\sigma_S)-\hat\sigma_S \bigr)  \ge \theta \sqrt{N} + \sum_{S\in\mathcal{S}}p_S\delta(S)\Bigr)\\
%     &\le \exp{\left(-\frac{2N{\Bigl(\theta + \frac{1}{\sqrt{N}}\sum_{S\in\mathcal{S}}p_S\delta(S)\Bigr)}^2}{\sum_{S\in\mathcal{S}} {(M_S - m_S)}^2}\right)}\;.
%   \end{aligned}
% \end{equation*}
% Consequently, we obtain
% \begin{equation*}
%     \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr)
%     \le 2 \exp{\left(-\frac{2N{\Bigl(\theta - \frac{1}{\sqrt{N}}\sum_{S\in\mathcal{S}}p_S\lvert \delta(S)\rvert \Bigr)}^2}{\sum_{S\in\mathcal{S}} {(M_S - m_S)}^2}\right)}\;,
% \end{equation*}
% which is insightful, provided that
% $\theta > \frac{1}{\sqrt{N}}\sum_{S\in\mathcal{S}}p_S\lvert
% \delta(S)\rvert$. The connection to the failure probability derived
% before becomes apparent, when considering a relative error by setting
% $\theta = \tau \sqrt{\mathcal{V}} = \frac{\tau}{\sqrt{N}}\varsigma
% $. In that case the preceding display yields
% \begin{equation*}
%   \mathbb{P}\Bigl(\bigl\vert \sqrt{\hat{V}} - \sqrt{\mathcal{V}} \bigr\vert \ge \theta \Bigr) =
%   \mathbb{P}\bigl(\lvert R - 1 \rvert \ge \tau \bigr)
%     \le 2 \exp{\left(-\frac{2{\Bigl(\tau\varsigma - \sum_{S\in\mathcal{S}}p_S\lvert \delta(S)\rvert \Bigr)}^2}{\sum_{S\in\mathcal{S}} {(M_S - m_S)}^2}\right)}\;,
% \end{equation*}
% Comparing that bound with the one in
% \eqref{eq:failure:prob:global:hoeffding:rel:final}, we notice that the
% only difference in the denominators. In fact, the upper bound in
% \eqref{eq:failure:prob:global:hoeffding:rel:final} will be smaller due to
% the weighted average ($0\le p_S\le 1$).
%}

\subsection{Probability of a catastrophic failure}
So far we have quantified the probability that the estimated variance
of the stratification estimator differs significantly form its true
variance. However, using the same arguments as before we can also
derive an upper bound on the ``catastrophic'' failure that the
estimated variance of the stratification estimator even exceeds the
variance of the classic Monte Carlo estimator. That is, let
$R^{\text{mc}} := \sqrt{\hat{V}/\mathcal{V}^{\text{mc}}}$ denote the
ratio of the estimated standard deviation and the standard deviation
of the Monte Carlo estimator using $N$ samples, which is given by
$\mathcal{V}^{\text{mc}} = N^{-1}\var{f(\boldsymbol{X})} \equiv
\sigma^2/N$. The catastrophic failure probability of
$R^{\text{mc}}\ge \rho$ for some suitable $\rho>0$ is thus bounded by
\begin{equation}\label{eq:failure:prob:catastrophic}  
    \mathbb{P}\bigl(R^{\text{mc}}\ge \rho \bigr) = \mathbb{P}\Bigl( \sum_{S\in\mathcal{S}} p_S\hat\sigma(S)\ge \rho \sigma \Bigr)
    \le\exp{\left(-\frac{2{\left(\sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert - (\rho\sigma - \varsigma)\right)}^2}{\sum_{S\in\mathcal{S}} {p_S}^2{(M_S - m_S)}^2}\right)}\;,
\end{equation}
provided that
\begin{equation*}
  \rho > \frac{\varsigma + \sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert}{\sigma} = 1 - \frac{\sigma - \varsigma - \sum_{S\in\mathcal{S}} p_S \lvert\delta(S)\rvert}{\sigma} \;.
\end{equation*}
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Master"
%%% End:
